Forecasting Time Series with VARMA Recursions on Graphs

Graph-based techniques emerged as a choice to deal with the dimensionality issues in modeling multivariate time series. However, there is yet no complete understanding of how the underlying structure could be exploited to ease this task. This work provides contributions in this direction by considering the forecasting of a process evolving over a graph. We make use of the (approximate) time-vertex stationarity assumption, i.e., timevarying graph signals whose first and second order statistical moments are invariant over time and correlated to a known graph topology. The latter is combined with VAR and VARMA models to tackle the dimensionality issues present in predicting the temporal evolution of multivariate time series. We find out that by projecting the data to the graph spectral domain: (i) the multivariate model estimation reduces to that of fitting a number of uncorrelated univariate ARMA models and (ii) an optimal low-rank data representation can be exploited so as to further reduce the estimation costs. In the case that the multivariate process can be observed at a subset of nodes, the proposed models extend naturally to Kalman filtering on graphs allowing for optimal tracking. Numerical experiments with both synthetic and real data validate the proposed approach and highlight its benefits over state-of-the-art alternatives.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> journal revised/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> journal revised/section_conclusion.tex <==
% !TEX root = main.tex

%
The purpose of this work was to determine multivariate models for forecasting the temporal evolution of time series on graphs. 
%
%It used recent findings in time-vertex signal processing and showed that the prediction accuracy improves by incorporating the underlying structure into the multivariate VAR and VARMA recursions. 
By leveraging the (approximate) joint time-vertex stationary of the time series, we reduced the DoFs for the VAR and VARMA models by designing their coefficients in the graph spectral domain. The latter decomposition allowed us to fit the model parameters with well-known univariate techniques by tackling both the computational and stability issues present in classical VAR and VARMA models. To further reduce the estimation costs, we proposed an optimal low-rank representation for the time series. Finally, a sub-graph tracker was introduced when measurements form a subset of nodes become available.
%

The findings clearly indicated that the graph structure plays a major role in easing the computational complexity of high dimensional multivariate models. This role is further enhanced when the amount of training data is limited. %with limited training data.
%
Several numerical experiments showed the benefits of the proposed methods over the classical multivariate forecasting techniques and other the state-of-the-art graph-based approaches.

Overall, this work strengthens the idea that practical benefits could be achieved in the time series forecasting if the underlying data connections are exploited. Further work is needed in two main directions. First, it is important to understand the implications of the stationary assumption for the task of prediction. Second, it is useful to analyze the effects of the graph structure in the prediction accuracy.


==> journal revised/section_fitting.tex <==
%!TEX root = main.tex

In this section, we focus on identifying the model parameters, \ie the kernel matrices $a_p(\L_\Gr)$ and $b_q(\L_\Gr)$ for the G-VARMA, or the scalars $\psi_{l,p}$ for the GP-VAR, that fit process $\X_{1:T}$. We start with the more complex G-VARMA case and introduce a GFT-based decoupling approach to ease the computational burden. To further reduce the parameter estimation costs, we introduce a low-rank model which trades prediction accuracy with computational complexity. Then, we consider the GP-VAR predictor and show that the scalar parameters can be estimated from the graph process statistics. The section is concluded with the notion of joint frequency smoothing and its application to parameter design.

%---------------------------------------------------------------------------------------------------
%---------------------------------------------------------------------------------------------------
\subsection{G-VARMA fitting}
\label{subsec_cgvarma}

Given the realizations $\X_{1:T}$, the canonical way for estimating the kernel matrices $a_p(\L_\Gr)$ and $b_q(\L_\Gr)$ is by solving

\begin{equation}
\label{eq.gcvarma_estim}
\minimize_{a_p(\L_\Gr), b_q(\L_\Gr)} \sum_{\tau = \text{max}\{P,Q\}}^{T-1}\bigg\|\x_\tau - \tilde{\x}_{\tau}[a_p(\L_\Gr), b_q(\L_\Gr)]	\bigg\|_2^2.\\
\end{equation}
%
{Problem~\eqref{eq.gcvarma_estim} involves a non-linear system of $N \times (T-1- \text{max}\{P,Q\})$ equations with $(P+Q)N$ unknowns whose computational complexity can become prohibitive even for moderate values of $N$ and $T$.
%
%
 %for general kernel matrices $a_p(\L_\Gr)$, $b_q(\L_\Gr)$, or $(P+Q)N$ unknowns for kernel matrices that represent graph filters, \ie $a_p(\L_\Gr) = \U_\Gr a_p(\LAM_\Gr)\U_\Gr^\herm$, $b_q(\L_\Gr) = \U_\Gr b_q(\LAM_\Gr)\U_\Gr^\herm$. In both instances, the computational complexity of solving \eqref{eq.gcvarma_estim} can be prohibitive, even for moderate values of $N$ and $T$.
%
To alleviate these costs, the following proposition establishes a decoupling approach that breaks down problem \eqref{eq.gcvarma_estim} into $N$ uncorrelated (yet not equivalent) well-studied problems with smaller complexity.}

\begin{proposition}[Decoupling]\label{prop.decoup} Consider the joint causal model~\eqref{eq:joint_causal_model}
%
\begin{align*}
\x_t = -\sum_{p = 1}^P a_p(\L_\Gr) \, \x_{t-p} +  \sum_{q = 0}^Q b_{q}(\L_\Gr) \, \eps_{t-q},   
    %\label{eq:prop1}
\end{align*} 
%
and denote with $\hat{\varepsilon}_{t,n} = [\U_\Gr^{\herm} \eps_{t}]_n$ and $\hat{x}_{t,n} = [\U_\Gr^{\herm} \x_{t}]_n$ the $n$th GFT coefficient of $\eps_{t}$ and $\x_{t}$, respectively. Then, the input-output relation between $\hat{\varepsilon}_{t,n}$ and $\hat{x}_{t,n}$ is given by the ARMA recursion 

%$\sum_{p = 0}^P a_p(n) \hat{x}_{t-p}(n)  = \sum_{q = 0}^Q b_q(n) \, \hat{\varepsilon}_{t-q}(n)$
\begin{align}
     \hat{x}_{t,n} = - \sum_{p = 1}^P \left[a_p(\LAM_\Gr)\right]_{n,n} \hat{x}_{t-p,n} + \sum_{q = 0}^Q \left[b_q(\LAM_\Gr)\right]_{n,n} \, \hat{\varepsilon}_{t-q,n},
    \label{eq:prop2}
\end{align} 
% 
with $\left[b_0(\LAM_\Gr)\right]_{n,n} = 1~\forall n$ and $n = 1, \ldots, N$.
\end{proposition}

(The proof is given in the Appendix.)

Although simple in its derivation, Proposition \ref{prop.decoup} relates different aspects of the graph and the time series with the model fitting. First, it uses the GFT eigenbasis to formulate \eqref{eq:joint_causal_model} in the graph Laplacian eigenspace\footnote{Recall that for JWSS graph processes the eigenvectors $\U_\Gr$ of $\L_\Gr$ coincide with the eigenvectors of $\bSigma_x$.}. Second, the model fitting is performed in the graph frequency domain. Here, the parameter estimation is split into $N$ uncorrelated problems of a smaller complexity involving $T$ equations and $P+Q$ unknowns. Despite being non-linear problems, the estimation for each graph frequency time series results in fitting a univariate temporal ARMA. So, we can use well-studied methods to solve it, such as the Gauss-Newton approach \cite{wills2008gradient}. 

\begin{remark}[Estimation cost]
In our analysis, the eigendecomposition of the graph Laplacian $\L_\Gr$ is crucial to estimate the G-VARMA parameters. Therefore, the proposed framework suits better small to medium-sized graphs, where the eigenvalue decomposition cost (inherent in joint models), is overshadowed by that of the model estimation. Nevertheless, next, we introduce a low-rank model estimation that reduces the estimation complexity at the expense of fitting accuracy.
\end{remark}

\noindent\textbf{Low-rank models.}  To further reduce the model estimation cost, we can consider estimating $a_p(\L_\Gr)$ and $b_q(\L_\Gr)$ only from a subset of graph frequencies, say $K \le N$. The latter incurs considerable savings in terms of estimation complexity since $(i)$ there is no need to compute the full eigendecomposition of $\L_\Gr$, but only the eigenvectors relative to the chosen $K$ graph frequencies; and $(ii)$ we only need to fit $K \le N$ temporal ARMA time series to the data. For this purpose, we use the following definition of low-rank matrix approximation.

\begin{definition}[Low-rank approximation] Let $\Scal$ be an index set of cardinality $K = |\Scal|$, with indicator matrix $\D_\Scal$. Let also $\U$ be a unitary (rotation) matrix. The $\{\U, \Scal\}$ low-rank approximation of a matrix $\X_{1:T}$ is
\begin{equation}
\tilde{\X}_{\U,\Scal} = \U\D_\Scal\U^\herm\X_{1:T}.
\end{equation}
\end{definition}
For prediction, which is an online task, the above low-rank approximation should be done only w.r.t. the graph dimension. %On the other hand, for offline regression tasks, a low-rank approximation can also be considered in the time-dimension. 
The following theorem provides a constructive way to design the set $\Scal$ that achieves the \emph{optimal low-rank} approximation for a JWSS process.

\begin{theorem}\label{theo.low_rank}
Let $\X_{1:T}$ be a zero-mean JWSS process. The optimal K-rank approximation of $\X_{1:T}$ is given by
\begin{equation*}
\label{eq.theo_LR}
\{\U_\Gr,\Scal^\star	\} = \argmin_{\U, \Scal}\Exp\left[	\left\|	\X-\tilde{\X}_{\U,\Scal}	\right\|^2_F	\right]\quad \text{s.t.}\quad |\Scal| = K,
\end{equation*}
where $\Scal^\star$ contains the indices of the $K$ largest diagonal elements of $\U_\Gr^\herm\bSigma_{x}\U_\Gr$.% $\U_\Gr^\herm\Exp\left[\X_{1:T}\X_{1:T}^\herm	\right]\U_\Gr$.
\end{theorem}

(The proof is given in the Appendix.)

This result suggests that the best rank$-K$ approximation of $\X_{1:T}$ is obtained by rotating the JWSS process by the graph Laplacian eigenvectors. This finding is beneficial since the first step in the model estimation consists of decoupling the time series using the GFT. It further allows us to claim the following:


%Theorem~\ref{theo.low_rank} implies that the best K-rank approximation of $\X_{1:T}$ is obtained by rotating the JWSS process by the graph Laplacian eigenvectors $\L_\Gr$. The latter is beneficial to us, since the first step in the model estimation is by decoupling the time-series with the GFT. This finding leads to the following corollary.

\begin{corollary}\label{cor_transf} Let $\U_{\Gr,K}$ denote the $N \times K$ matrix containing the $K$ columns of $\U_\Gr$ relative to the $K$ {highest} eigenvalues of $\bSigma_x$. Then, $\U_{\Gr,K}^\herm\bSigma_{x}\U_{\Gr,K}$ leads to the same result as selecting the {highest} K diagonal elements of $\U_\Gr^\herm\bSigma_{x}\U_\Gr$.
\end{corollary}
%(The proof can be derived with simple algebra.)

An important outcome of the last two results is that the full eigendecomposition of $\L_\Gr$ is not needed. Indeed, only the eigenvectors relative to the $K$ largest eigenvalues of $\bSigma_{x}$ are needed (recall that $\U_\Gr$ jointly diagonalizes both $\L_\Gr$ and $\bSigma_{x}$), which can be obtained with a lower cost.
% Indeed only the eigenvectors relative to the $K$ \textcolor{red}{highest} eigenvalues are needed, which can be obtained with a much lower cost. 
Therefore, the low-rank representation can be combined with the model estimation, by only modeling the time series for the graph frequencies in $\Scal$. In this way, we attain a reduction in the model estimation cost of $N/K$ allowing the G-VARMA to cope well with largely-sized graphs.
%
Later in Section~\ref{subsec_lowRank}, we will see that real data enjoy this low-rank representation with $K \ll N$.

%In our numerical tests, we show that real data often have this low-rank representation where $K$ is generally small. Therefore, a significant complexity reduction in the parameter estimation is obtained allowing the methods to cope well with large sized graphs.

\begin{figure*}[!b]
\hrulefill
%\begin{strip}
\begin{align}
\begin{split}
&\underset{\{\psi_{l,p}\}}{\text{minimize}}\quad \trace\left(\R_x(0)	 +\sum_{p=1}^P\bPsi_p\R_x(p) +\sum_{p=1}^P\R_x(p)\bPsi_p^\herm + \sum_{p_1 = 1}^P\sum_{p_2 = 1}^P\bPsi_{p_1}\R_x(p_2-p_1)\bPsi_{p_2}^\herm\right)\\
&\text{subject to} \quad \bPsi_p = \sum_{l=0}^{L_p}\psi_{l,p}\L_\Gr^l.
\end{split}
\label{eq.gc_varprob}
\end{align}
%\end{strip}
\end{figure*}

%---------------------------------------------------------------------------------------------------
%---------------------------------------------------------------------------------------------------
\subsection{GP-VAR fitting}
\label{subsec_cgpvar}

The parameter estimation for the GP-VAR model \eqref{eq.gcp_varma} consists of estimating the scalars $\psi_{l,p}$. Since this problem has a lower complexity, we find the $\psi_{l,p}$ coefficients by directly minimizing the prediction MSE
%
\begin{equation}
\label{eq.gcp_MSE1}
\text{MSE} = \Exp\Bigg[\Bigg\|\x_t + \sum_{p=1}^P\bPsi_p\x_{t-p} 	\Bigg\|_2^2\Bigg],
\end{equation}
with $\bPsi_p = \sum_{l=0}^{L_p}\psi_{l,p}\L_\Gr^l$. From $\|\x\|_2^2 = \trace(\x\x^\herm)$ and the linearity of the trace and the expectation, \eqref{eq.gcp_MSE1} becomes
%
\begin{align}
\label{eq.gcp_MSE2}
\begin{split}
\text{MSE} &= \trace\left(\sum_{p=1}^P\bPsi_p\Exp\left[ \x_{t-p}\x_t^\herm	\right]	\right) + \trace\left(\sum_{p=1}^P\Exp\left[\x_t\x_{t-p}^\herm\right]\bPsi_p^\herm\right)\\
&\hskip-.6cm+\trace\left(\Exp\left[\x_t\x_t^\herm	\right]	\right) + \trace\left(\sum_{p_1 = 1}^P\sum_{p_2 = 1}^P\bPsi_{p_1}\Exp\left[\x_{t-p_1}\x_{t-p_2}^\herm\right]\bPsi_{p_2}^\herm\right)\!. %+ \trace\left(\sum_{q_1 = 0}^Q\sum_{q_2 = 0}^Q\bPhi_{q_1}\Exp\left[\eps_{t-q_1}\eps_{t-q_2}^\herm\right]\bPhi_{q_2}^\herm\right)\\
\end{split}
\end{align}
Then, since $ \R_x(i) = \Exp[\x_t\x_{t-i}]$ is the autocorrelation of the process at lag $i$, the GP-VAR coefficients can be found by solving the convex problem \eqref{eq.gc_varprob}.


%
%Differently from the CG-VARMA model, the coefficient estimation \eqref{eq.gc_varprob} is now a convex problem and can be solved efficiently with of-the-shelf optimization tools such as CVX \cite{grant2008cvx}. 

From \eqref{eq.gcp_MSE1}-\eqref{eq.gc_varprob}, the graph topology imposes a structure on the model coefficients. In fact, this, somehow small, modification renders the model parameter estimation a computationally easier task compared to the classical VAR model. Thus, more robust to cope with larger multivariate dimensions. The GP-VAR model inherits several benefits from the classical literature of multivariate VAR analysis \cite{lutkepohl2005new}. In \eqref{eq.gc_varprob}, we rely on the autocorrelation matrix to estimate the coefficients, which must be estimated from the training data $\X_{1:T}$, \ie $\R_x(i) = (T-i)^{-1}\sum_{\tau=0}^{T-i}\x_\tau\x_{\tau+i}^\herm$. Differently from \cite{di2016adaptive, di2017adaptive, Qiu2017, romero2016kernel} that do not exploit stationary assumptions, in the GP-VAR model we can incorporate well-established techniques for estimating $\R_x(i)$, such as the shrinkage estimators \cite{ledoit2004well} and the random matrix theory-based estimator \cite{tulino2004random} in low-samples regime, or the Kullback-Leiber divergence \cite{sun2014regularized} and Tyler's estimator \cite{tyler1987distribution} to deal with heavy tail issues in non-Gaussian scenarios.

\begin{remark}[Yule-Walker estimation] An alternative to \eqref{eq.gc_varprob} for estimating $\psi_{l,p}$ is to follow a Yule-Walker approach \cite{Hayes2009}. That is, minimize in a least squares sense the function $f(\psi_{l,p}) = \R_x(0) + \sum_{p = 1}^P\bPsi_p\R_x(p)$ with $\bPsi_p = \sum_{l=0}^{L_p}\psi_{l,p}\L_\Gr^l$. Besides being a computationally lighter problem to solve, the Yule-Walker strategy can be combined with the approach in \cite{chepuri2017graph} and, thus, estimate the $\psi_{l,p}$ from subsampled measurements.
\end{remark}
%
%
%Additionally, from \eqref{eq.gc_varprob} we observe that the model estimation follows the classical VAR models \cite{lutkepohl2005new} with the graph that imposes a particular structure on model coefficients. There is yet a practical aspect concerning the CGP-VAR model \eqref{eq.gcp_varma} to consider. Specifically, in \eqref{eq.gc_varprob} we rely on the autocorrelation matrix to estimate the coefficients.  Generally, this information is not given to us and it should be estimated from the training data $\X_{1:T}$, \ie $\R_x(i) = (T-i)^{-1}\sum_{\tau=0}^{T-i}\x_\tau\x_{\tau+i}^\herm$. In fact, differently from \cite{di2016adaptive, di2017adaptive, Qiu2017, romero2016kernel} that do not exploits stationarity assumptions, the latter allows our model to incorporate well-established techniques for estimating $\R_x(i)$, such as shrinkage estimators \cite{ledoit2004well}, random matrix theory-based estimator \cite{tulino2004random} in low-samples regime, or Kullback-Leiber divergence \cite{sun2014regularized} and Tyler's estimator \cite{tyler1987distribution} for dealing with heavy tail issues in non-Gaussian scenarios.

%---------------------------------------------------------------------------------------------------
%---------------------------------------------------------------------------------------------------
\subsection{Spectral Smoothing}
\label{subsec_specSmooth}
%\textcolor{red}{Some comments here: i) I changed $\omega$ to $e^{-\j\omega}$ for consistency with Sec. II. ii) For my understanding: (23) is a separable function in the joint frequency domain right? In that case, one can also say we first do smoothing on the graph frequencies and then on the temporal frequencies. iii) I modified a bit the final explanantion of this. It was to much oriented on the graph smoothing and on a general viewpoint. Since, this is already proposed, in this work I prefer to stick to its benefits w.r.t. our problem. The previous writing is commented in latex.}

We can further improve the model fitting by using the spectral smoothing heuristic \cite[Section IV. B]{loukas2016stationary}. This involves the convolution of the JPSD with a smoothly decaying windowed function in the spectral domain. Specifically, if $\P_{1:T} = |\JFT{\X_{1:T}}|^2$ is the JPSD in matrix form, we fit the models to the process having a final JPSD
%
\begin{align}\label{eq.spec_smooth}
	[\tilde{\P}_{1:T}]_{\lambda, e^{-\j\omega}} \!=\!\! \sum_{n,t} g_{\mathcal{G}}(\lambda \!-\! \lambda_n)^2\! g_{\mathcal{T}}(e^{-\j\omega} \!-\! e^{-\j\omega_t})^2 \,\! [\P_{1:T}]_{\lambda_n, e^{-\j\omega_t}},
\end{align}
%
where $g_{\mathcal{G}}$ and $g_{\mathcal{T}}$ are smoothly decaying functions in the graph and temporal and frequency domains, respectively. 
$g_\Gr$ and $g_{\mathcal{T}}$ are scaled Gaussian functions centered at zero and normalized to sum to one. The Gaussian width is a free parameter that controls the estimator's bias-variance trade-off~\cite{loukas2016stationary}.%\elvin{Instead of this wordy explanation, an expression for $g_{(\cdot)}$ would be better specifying visually the tuning parameter.}\andreas{Let us leave it like this.}

The idea of spectral smoothing is common in time series analysis. In fact, for stationary time series, spectral smoothing (i.e., the convolution with $g_{\mathcal{T}}$ along each node) is a technique encountered in the literature (see \cite{bartlett1950periodogram,welch1967use}).
%
For stationary graph signals, spectral smoothing w.r.t. the graph Fourier domain (i.e., the convolution with $g_{\mathcal{G}}$ along each $t$) is used to better estimate stationary graph signals~\cite{Perraudin2016, girault2017towards}.
%
This heuristic also relates to the spectral leakage phenomenon in eigenvalue estimation~\cite{loukas2017close}, exploiting the locality of spectral leaking to better estimate the eigenvalues of the covariance matrix from few samples.
%

With respect to this work, \eqref{eq.spec_smooth} relates the joint stationarity of the signal with the challenge of estimating the model parameters in a low sample regime. This heuristic exploits the fact that the signal JPSD is likely to have similar values in adjacent frequencies and that abrupt changes are more likely to occur due to noise and finite sample estimation inaccuracies. Therefore, by exploiting the latter, a model fitting to data with a JPSD as in \eqref{eq.spec_smooth} will often lead to a lower estimation error.

  
%For wide-sense stationary timeseries, spectral smoothing (i.e., convolution with $g_T$ along each $n$) is a technique commonly encountered in the literature. Bartlett and Welch~\cite{bartlett1950periodogram,welch1967use} for instance use it to decrease the estimation variance by promoting localization of the auto-correlation in the frequency domain.
%
%Spectral smoothing with respect to the graph eigenvalue domain (i.e., convolution with $g_G$ along each $t$) was first utilized for estimating graph stationary signals by Perraudin and Vandergheynst~\cite{Perraudin2016} and later on by Girault et al.~\cite{girault2017towards}. Graph spectral smoothing can be interpreted as promoting the localization of the auto-correlation in the graph domain. 
%
%The heuristic also relates to the spectral leaking phenomenon in eigenvalue estimation~\cite{loukas2017close}. When the number of samples used to estimate the covariance matrix is small, there is poor separation between eigenspaces resulting in a miscalculation of the PSD. However, any occurring errors are strongly localized, meaning that the power in each subspace leaks only to nearby subspaces. The spectral smoothing heuristic exploits this phenomenon in order to reduce the estimation variance.


%\andreas{maybe add a table with model names, number of parameters, evaluation complexity, method for training, and perhaps assumptions?}\elvin{Elvin: I really like the idea. I'll see in the very end if we have space. If not, we can send it as supplementary material and then add it in the next revision round.}










==> journal revised/section_intro.tex <==
%!TEX root = main.tex

Forecasting multivariate processes is a central topic in signal processing \cite{box2015time,lutkepohl2005new}. Especially in the high-dimensional setting, the forecasting of \emph{unstructured data} is considered a complex task, both from an estimation and computational perspective --indeed, most works in this direction stay within the limit of a few dozen time series. To cope with the dimensionality challenge, particularly when the number of observations is smaller than the number of time series, typical solutions involve factor models \cite{connor1995three,lam2011factor}, shrinkage estimators \cite{meucci2009risk,ledoit2004well}, and low-rank data representations \cite{lutkepohl2005new}.

Recently, forecasting has been considered for \emph{graph-structured} processes, i.e., time-varying signals living on the nodes of graphs~\cite{mei2017signal,di2016adaptive,di2017adaptive,Qiu2017,romero2016kernel}. Here, given a graph and a set of time series, the aim is to exploit the underlying structure for improving the prediction accuracy of the considered model. The core idea is that the additional information, carried by the graph, can enhance our ability to make relevant predictions. The graph basically aids to restrict the degrees of freedom (DoFs) of the model in a manner faithful to the problem at hand. Depending on the scenario, these works exploit different signal priors w.r.t. the graph to formulate the prediction task. 

The first to consider prediction in the graph context is the work of~\cite{mei2017signal}, which used the vector autoregressive (VAR) recursions to learn the underlying topology and then used this structure to forecast future values. Their findings rely on a temporal interpretation of edges. More specifically, it is assumed that the information requires a unit time step to reach adjacent nodes. 
Coupling the duration of graph interactions and the fixed temporal resolution in such a manner may be beneficial for graph learning purposes, but negatively affects forecasting since it ignores hidden correlations between nodes.

Relevant work has also been done in \emph{tracking} time-varying signals on graphs\footnote{For the sake of clarity, the reader should distinguish between forecasting and tracking a time-varying signal. In forecasting, $x_t$ is predicted based on historical data $\{x_0, \ldots, x_{t-1}\}$, while in tracking noisy measurements at time $t$ are also used.}. In the adaptive approaches~\cite{di2016adaptive,di2017adaptive}, the prediction/tracking of time-varying graph signals comes as a byproduct of the presented adaptive estimation strategies. Here, the authors exploit a low-rank representation of the signal, due to the bandlimitedness in the graph spectral domain, to track slow signal variations over time. 

A different approach for network process tracking is followed in \cite{Qiu2017,romero2016kernel}. Here, a virtual graph extrapolated to the temporal dimension is considered and the multivariate time series is treated as a single time-invariant (extended) graph signal on this larger graph. Then, under priors such as diffusion or smoothness, the tracking task is rephrased as an interpolation problem. To ease the excessive computational burden, gradient descent algorithms \cite{Qiu2017} or Kalman-based recursions \cite{romero2016kernel} are invoked.

Almost all the above works treat the time series as the evolution of a noise-corrupted deterministic process. However, in many practical situations including opinion blogs, temperature sensor networks, financial markets, or brain networks, the time series has a strong stochastic component. The latter requires models able to capture the stochasticity along both the graph and time dimension and allow the short time prediction from few training samples. Some earlier contributions have considered stochasticity in time, see e.g., \cite{mei2017signal,di2017adaptive}, yet leaving unexplored the stochasticity along the graph dimension.

This work takes one step further and treats time series as wide-sense stationary (for short stationary) statistical processes w.r.t. both the graph and temporal domains. While temporal stationarity preserves the process statistics w.r.t. translations in time, the considered joint stationarity hypothesis also preserves these statistics w.r.t. graph localization. \rev{A typical example comprises temperature measurements in sensor networks. The graph stationarity implies that neighboring sensors yield in expectation a constant value. The joint stationary, on the other hand, considers the expected constant value to be also preserved in consecutive time instances}\footnote{We remark that although perfect stationarity either in the time or graph domain is difficult to be observed, several real data sets \cite{Girault2015,Perraudin2016,Marques2016,loukas2016stationary} have shown some degree of graph/time stationarity that can be exploited for prediction.}.

Continuing our prior works \cite{loukas2016stationary,Isufi2016separable}, we exploit the (approximate) time-vertex stationarity of graph time series and extend classical VAR and vector autoregressive moving average (VARMA) recursions for modeling and predicting time-varying processes on graphs. Specifically, the contributions of this work are:
%
\begin{enumerate}
\vskip1mm
\item We propose VAR and VARMA models for forecasting time series on graphs. These recursions extend the non-causal models of \cite{loukas2016stationary} to causal ones and generalize the approach of \cite{mei2017signal} to $(i)$ VAR recursions that do not impose a temporal interpretation of the edges, and $(ii)$ VARMA recursions where the MA part allows to model time series with a more complete structure. 
%\vskip1mm
%\item We incorporate the notion of time-vertex stationarity to extend the non-causal models of \cite{loukas2016stationary} to causal recursions on graphs. The proposed graph VAR and VARMA models generalize the approach of \cite{mei2017signal} to $(i)$ VAR recursions that do not impose a temporal interpretation of the edges capturing more hidden correlations between nodes, and $(ii)$ VARMA recursions where the MA part allows to model time series with more complicated structure. 
\vskip1mm
\item We propose a model fitting method that makes use of the data structure and stationarity. % through the so-called graph Fourier transform (GFT) \cite{Shuman2013}. 
Specifically, we separate the multivariate process into uncorrelated univariate time series (one per graph frequency), hence tackling the dimensionality issue present in VARMA modeling. The latter enables us to use well-established univariate techniques for estimating the model coefficients from limited training data. We further introduce an optimal low-rank data representation, which intrinsically makes use of the graph to further reduce the computational overhead of the model estimation.
%Specifically:
%\begin{enumerate}
%\vskip1mm
%\item Through the GFT, we separate the multivariate process into independent univariate time series (one per graph frequency), and, hence, tackle the dimensionality issue present in VARMA modeling. This also enables us to use well-established univariate techniques for estimating the model parameters from limited training data.
%%\item  We bring forth a decoupling approach that allows us to separate the multivariate process into independent univariate time series (one per graph frequency), and, hence, tackle the dimensionality issue present in multivariate forecasting. Furthermore, this decoupling approach entails us to use classical and well-established univariate techniques for estimating the model parameters from few training data.
%\vskip1mm
%\item We introduce an optimal low-rank approximation of the training data, which intrinsically makes use of the graph structure to further reduce the computational overhead of model estimation.
%%
%%\item We introduce an optimal low-rank approximation of the training data, which intrinsically makes use of the graph structure to further reduce the computational overhead of model estimation. The latter allows us to estimate the model parameters from a subset of the graph frequencies and thus, reducing proportionally the parameter estimation costs. %\textcolor{red}{Elvin: No spectral smoothing here?} \andreas{It turns out it was done before, so I didn't want to stress it.}
%%\item \textcolor{red}{TO DO: Spectral Smoothing.}
%\end{enumerate}
\vskip1mm
\item We introduce a sub-graph tracker to estimate the time series on a subset of nodes. The latter makes use the prediction at time $t$ along with graph sub-sampled measurements to estimate the attributes on the nodes of interest. We show a direct connection between the proposed approach and Kalman filtering (KF) on graphs \cite{isufi2017observing} that allows a direct characterization of the sub-graph tracker performance. %Yet, there is a fundamental difference between the two: The proposed sub-graph tracker considers none model evolution of the signal, rendering it more versatile to non-diffusive phenomena.
%
%\item We introduce a sub-graph predictor to track the time series' value at a subset of nodes. Our algorithm uses the prior evolution of the data along with some graph sub-sampled measurements to find the attributes on the unobserved nodes. Two typical scenarios of the latter include: $(i)$ the opinion evolution on a network, where some of the users (vertices) do not take part in the survey after a certain time instant; and $(ii)$ the signal evolution on a sensor network, where due to energy constraints some sensors may not be sampled after a given time. While in the first scenario the sampled vertices are fixed by the problem, in sensor networks we can carefully sample the right sensors that yield an improved prediction accuracy. We demonstrate how this task can be effectively addressed with the proposed joint causal models, where a detailed MSE analysis highlights the role played by the sampling set and the graph topology. An important consequence is that the position of the sampled nodes w.r.t. the graph is as important as the cardinality of the sampling set, enforcing the idea that the prediction task is highly influenced by the graph topology. We finally propose a sparse sensing-based technique to sample the graph given a target prediction MSE cost.
\end{enumerate}
%
The paper makes an additional minor contribution. It generalizes the separable two-dimensional time-vertex ARMA filter of \cite{Isufi2016separable} to a non-separable version and shows that the latter encompasses other state-of-the-art time-vertex recursions on graphs as the ones presented in \cite{mei2017signal,Isufi2016Dim2} and can be used for distributed predictors.

To validate the joint stationarity hypothesis and the proposed models, we consider three scenarios: $(i)$ {the Molene weather} data set\footnote{\rev{Data publicly available at \texttt{https://donneespubliques.\\meteofrance.fr/donnees\_libres/Hackathon/RADOMEH.tar.gz}.}}; the NOAA U.S. temperature data set \cite{nooaDataset} $(ii)$ a dynamic mesh data set containing a walking dog; and $(iii)$ an epidemic spreading scenario over a flight transportation network. The obtained results corroborate the relevance of graph VARMA models for forecasting stochastic time series supported on graphs and show that the proposed approaches outperform both classical univariate and multivariate ARMA techniques and state-of-the-art graph-based techniques. 

 %$(ii)$ a simulated epidemic spreading over the flight transportation network where the goal is to predict the percentage of infected individuals in 200 major European cities; and $(iii)$ a dynamic mesh data set depicting a walking dog, where the points position at consecutive frames should be predicted. 
%The obtained results show the proposed approach outperforms both classical univariate and multivariate ARMA techniques and state-of-the-art graph-based techniques in all datasets and settings. \andreas{Give a number here quantifying the improvement.} These experimental results corroborate the relevance of graph VARMA models for forecasting stochastic time series supported on a known graph topology.

\vskip1mm
\noindent\textbf{Notation.} The scalar $a_i$ indicates the $i$th entry of vector $\a$, and similarly the scalar $A_{i,j}$ indicates the $(i,j)$th entry of matrix $\A$. When needed these entries will also be denoted as $[\a]_i$, or $[\A]_{ij}$. $\A^\transp$, $\A^*$ and $\A^{\herm}$ are respectively the transpose, the element-wise conjugate, and the Hermitian of $\A$. $\|\a\|_p$ and $\|\A\|_p$ indicate respectively the $p$-th norm of $\a$ and $\A$, whereas $\|\A\|_F$ is the Frobenius norm of matrix $\A$. The trace of $\A$ is denoted as $\trace(\A)$ and $\A \otimes \B$ is the Kronecker product of the matrices $\A$ and $\B$. $\a = \text{diag}(\A)$ is the operation that stores the diagonal elements of $\A$ into the vector $\a$, and $\A = \text{diag}(\a)$ is a diagonal matrix containing the vector $\a$ in the main diagonal. \rev{The operation $\a = \text{vec}(\A)$ concatenates the columns of $\A$ in $\a$} and $\text{vec}^{-1}(\cdot)$ is the inverse operation. The $N \times N$ identity matrix is denoted as $\I_N$, the $N \times 1$ all ones vector as $\mathbf{1}_N$, and the $N \times 1$ all zeros vector as $\mathbf{0}_N$. \rev{For a set $\Scal \subseteq \{1, \ldots, N\}$, $|\Scal|$ is the set cardinality, and $\D_\Scal$ is an $N \times N$ diagonal matrix with $[\D_\Scal]_{ii} = 1$ if $i \in \Scal$ and zero otherwise.} To avoid confusion, we refer to \emph{causality} in the classical sense \cite{lutkepohl2005new}, i.e., an event happening at time $t$ is influenced only by events prior to $t$ independently of the graph dimension. We will refer to the notion of causality used by \cite{mei2017signal} as \emph{restricted causality}, being a subclass of the former.

\vskip1mm
\noindent\textbf{Paper organization.} Section~\ref{sec.back} contains the background information. Section~\ref{sec.mod} formulates the prediction problem in the graph signal processing (GSP) perspective and develops the optimal predictor. Section~\ref{sec.fit} focuses on the model parameter design.
The subgraph tracker is introduced and analyzed in Section~\ref{sec.subset}. Section~\ref{sec.numRes} contains the numerical results and the paper conclusions are drawn in Section~\ref{sec.concl}. %The proofs are collected in the appendix.










==> journal revised/section_model.tex <==
%!TEX root = main.tex

This section formulates the problem of modeling the temporal evolution of a JWSS network process. We start with a joint non-causal model and highlight its implementation issues. Then, we follow the classical literature of VARMA recursions \cite{lutkepohl2005new} to propose joint causal models for graph-time series. Finally, the optimal MSE predictor is derived.

%---------------------------------------------------------------------------------------------------
%---------------------------------------------------------------------------------------------------
\subsection{Joint Non-Causal Models on Graphs}
\label{subsec_jncmg}
%Following Definition~\ref{def.jwss}, 
A JWSS process $\x_{1:T}$ can be obtained through filtering of a random white process $\eps_{1:T} = \text{vec}(\E_{1:T})$ with a joint time-vertex filter \eqref{eq:def_joint_filtering} (recall Definition~\ref{def.jwss}). Specifically, we can model $\x_{1:T}$ with the \emph{joint non-causal model}
%
\begin{equation}
\label{eq.jncm}
a(\L_{\mathcal{J}})\x_{1:T} = b(\L_{\mathcal{J}})\eps_{1:T},
\end{equation}
where $\eps_{1:T}$ is the innovation vector, \ie a random vector with zero-mean and identity covariance matrix. The $NT \times NT$ matrices $a(\L_{\mathcal{J}}) = \U_{\mathcal{J}}a(\LAM_\Gr,\LAM_{\mathcal{T}})\U_{\mathcal{J}}^\herm$ and $b(\L_{\mathcal{J}}) = \U_{\mathcal{J}}b(\LAM_\Gr,\LAM_{\mathcal{T}})\U_{\mathcal{J}}^\herm$ represent arbitrary joint filters. From \eqref{eq.jncm} and the statistics of $\eps_{1:T}$, the JPSD of $\x_{1:T}$ is
%
\begin{equation}
\label{eq.jpsd_xT}
\p_{1:T} = \text{diag}\Bigg(|a(\LAM_\Gr,\LAM_{\mathcal{T}})|^{-2}|b(\LAM_\Gr,\LAM_{\mathcal{T}})|^2\Bigg)
\end{equation}
\rev{for an invertible matrix model $a(\L_{\mathcal{J}})$.}

Despite its generality, model \eqref{eq.jncm} presents several issues for the task of prediction. First, its computational complexity results in a heavy task even for moderate values of $N$ and $T$.
%
%
%scales with the number of nodes $N$ and the temporal observations $T$, rendering the forecasting a computationally heavy task even for moderate graph dimensions. 
\rev{Second, \eqref{eq.jncm} is not causal.} This is problematic for prediction where one needs to forecast the future in a timely manner from the process history. To accomplish these challenges, next we introduce \emph{joint causal models}, which ease the computational costs and model the JWSS graph process in a causal manner.

%---------------------------------------------------------------------------------------------------
%---------------------------------------------------------------------------------------------------
\subsection{Joint Causal Models on Graphs}
\label{subsec_jcmg}

In the following, we introduce two models for forecasting time series on graphs. 

\vskip 1mm
\noindent\textbf{Graph-VARMA model.} Similar to the multivariate case~\cite{lutkepohl2005new}, a joint causal model on graphs has the form
%
\begin{align}
\x_t = -\sum_{p = 1}^P a_p(\L_\Gr) \, \x_{t-p} +  \sum_{q = 0}^Q b_{q}(\L_\Gr) \, \eps_{t-q},   
\label{eq:joint_causal_model}
\end{align}
where the $N \times N$ matrices $a_p(\L_\Gr) = \U_\Gr a_p(\LAM_\Gr)\U_\Gr^\herm$, $b_0(\L_\Gr) = \I_N$, and  $b_q(\L_\Gr) = \U_\Gr b_q(\LAM_\Gr)\U_\Gr^\herm$ are graph filters and $\eps_t$ is a random vector with zero-mean and covariance matrix $\bSigma_\varepsilon$. %By setting $b_0(\L_\Gr) = \I_N$ one gets the canonical form of \eqref{eq:joint_causal_model}. 

Following the convention of time series analysis, we call the above model a graph-VARMA (G-VARMA) model. Nevertheless, we also refer to it as a joint causal model because (for sufficiently large $P$ and $Q$) \eqref{eq:joint_causal_model} can describe all causal JWSS processes.

%\andreas{I changed the implementation complexity to per-iteration complexity.}
\begin{remark}[G-VARMA complexity]
The per-iteration complexity of the G-VARMA model is $O((P+Q)N^2)$ amounting to $P+Q$ matrix-vector multiplications. 
\end{remark}

{In the sequel, we specialize model \eqref{eq:joint_causal_model} with graph filters $a_p(\L_\Gr)$ and $b_q(\L_\Gr)$ that have a polynomial structure over the graph. With the aim to implement a distributed predictor, we drop the MA part of \eqref{eq:joint_causal_model} and consider graph polynomial-VAR (GP-VAR) models. The rationale beyond the latter choice is that a graph polynomial VARMA model leads in practice to unstable predictors, or in best cases to predictors with larger MSE than GP-VAR. To some degree, this observation is not surprising and goes in line with the conclusions in multivariate modeling \cite[Chapter~11]{lutkepohl2005new}, \cite[Chapter~2]{feng2016signal}. Differently, this behaviour is not consistently observed for model \eqref{eq:joint_causal_model} due to its fitting procedure in the graph Fourier domain (see Proposition~\ref{prop.decoup} in Section~\ref{subsec_cgvarma}).}


\vskip 1mm
\noindent\textbf{Graph polynomial-VAR model.} By exploiting the proposed joint time-vertex filter \eqref{eq.2dARMA}, we write the matrices $a_p(\L_\Gr)$ and $b_{q}(\L_\Gr)$ as polynomials of the graph Laplacian $\L_\Gr$ and get the GP-VAR model\footnote{We denote the approach of \cite{mei2017signal} as restricted graph polynomial-VAR (RGP-VAR) model.}
%
\begin{equation}
\label{eq.gcp_varma}
\x_t = - \sum_{p = 1}^P\sum_{l = 0}^{L_p}\psi_{l,p}\L_\Gr^l\x_{t-p} + \eps_t%\varphi_{0,0}\eps_t,
\end{equation}
which is obtained from \eqref{eq:joint_causal_model} by setting $a_p(\L_\Gr) = \sum_{l = 0}^{L_p}\psi_{l,p}\L_\Gr^l$ for $p = 1, \ldots, P$ and $Q = 0$. \rev{Further, note that the order $L_p$ of the polynomials varies based on the time index.}


Model \eqref{eq.gcp_varma} preserves the recursive implementation of \eqref{eq:joint_causal_model}, thus it reduces further the computational complexity. The subsequent remark quantifies this cost.

\begin{remark}[GP-VAR complexity]\label{lemma.dist_complex} \rev{The Laplacian polynomial form of \eqref{eq.gcp_varma} allows it to be implemented distributively in the vertex domain with a complexity similar to \cite{Isufi2016separable}. By setting the maximum order of the Laplacian polynomial as $L_{\textit{max}} = max\{L_1, \ldots, L_p\}$, the per-iteration complexity of the GP-VAR model (13) is $O(L_{\textit{max}}|\mathcal{E}|)$.}
\end{remark}

%(The proof is given in Appendix~\ref{sec_appLemma}.)

Since in general $|\Ed| \ll N^2$, the (distributed) per-iteration computational complexity of the GP-VAR model \eqref{eq.gcp_varma} is much smaller than that of the G-VARMA model \eqref{eq:joint_causal_model}. Compared to the non-causal model \eqref{eq.jncm}, if we arrest the recursion after $T$ iterations, the computational complexity of the GP-VAR is $O(L_{\text{max}}|\Ed|T)$, while that of the G-VARMA is $O((P+Q)N^2T)$. Moreover, w.r.t. the RGP-VAR model of \cite{mei2017signal}, \eqref{eq.gcp_varma} allows the polynomial order in the graph domain $L_p$ to differ for each $p$ and not to be restricted as $L_p \le p$. The latter allows capturing more hidden interactions between nodes and, therefore, yields better predictors.
%
%
%Moreover, \eqref{eq.gcp_varma} generalizes the RGP-VAR model of \cite{mei2017signal}, where now the shifting order on the graph domain $L_p$ may vary for each $p$ and is not necessarily restricted to be $L_p \le p$. 
%
In Section~\ref{subsec_cgpvar}, we will see that this polynomial implementation simplifies the model design, to that of finding scalar coefficients rather than matrices as in \eqref{eq:joint_causal_model}. 

%We complete this section with the following observation.

%\begin{remark}[GP-VARMA] It is possible to extend model \eqref{eq.gcp_varma} so it accounts for the time-vertex history of the innovation signal $\eps_t$. This can be achieved by replacing $\eps_t$ with $\sum_{q = 0}^Q\sum_{k=0}^{K_q}\varphi_{k,q}\L_\Gr^k\eps_{t-q}$ in \eqref{eq.gcp_varma}. While the latter can be a choice, this model leads in practice to unstable predictors, or in best cases to predictors with larger MSE than the GP-VAR model. To some degree, this observation is not surprising and goes in line with the conclusions in multivariate modeling \cite[Chapter~11]{lutkepohl2005new}, \cite[Chapter~2]{feng2016signal}.
%\end{remark}

%---------------------------------------------------------------------------------------------------
%---------------------------------------------------------------------------------------------------
\subsection{Optimal predictor}
\label{subsec_pred}

Let $\X_{1:T}$ be the output of the more general G-VARMA model \eqref{eq:joint_causal_model}. We consider the realizations $\{\x_1, \ldots, \x_{t-1}\}$ are observed, and the goal is to estimate $\x_t$ from these values. Following the conventional approach \cite{lutkepohl2005new}, the value of $\x_t$ is estimated as the conditional expectation
%
\begin{align}\label{eq.one_stepPred}
\begin{split}
\tilde{\x}_t &= \Exp[\x_{t|t-1}]\triangleq \Exp\bigg[\x_t|\{\x_1, \ldots, \x_{t-1}\}\bigg]\\
&= - \sum_{p = 1}^P a_p(\L_\Gr)\, \x_{t-p} + \sum_{q = 0}^Q b_q(\L_\Gr) \Exp[{\eps_{t-q|t-1}}],
\end{split}
\end{align}
i.e., the expected value of $\x_t$ given the past realizations $\{\x_1, \ldots, \x_{t-1}\}$. Similarly, $\Exp[{\eps_{t-q|t-1}}]$ is the conditional expectation of $\eps_{t-q}$ given $\{\x_1, \ldots, \x_{t-1}\}$. Note that, since the past realizations $\{\x_1, \ldots, \x_{t-1}\}$ follow model \eqref{eq:joint_causal_model}, the knowledge of $\{\x_1, \ldots, \x_{t-1}\}$ allows computing the value of the \emph{specific realizations} for the past innovations $\{\eps_1, \ldots, \eps_{t-1}\}$ deterministically as $\eps_{t-q|t-1} = \x_{t-q|t-1} - \tilde{\x}_{t-q}$ for $q = 1, \ldots, Q$ (recall $b_0(\L_\Gr) = \I_N$). So, we can rewrite \eqref{eq.one_stepPred} as
%
\begin{align*}
\begin{split}
    &\tilde{\x}_{t} %&= \Exp[{ \x_{t|t-1} }]
    = - \sum_{p = 1}^P a_p(\L_\Gr) \x_{t-p}  + \b_0(\L_\Gr)\Exp[{\eps_{t}}] \\
    &\qquad\qquad\qquad + \sum_{q = 1}^Q b_q(\L_\Gr)\left(\x_{t-q|t-1} - \tilde{\x}_{t-q}\right)
\end{split}
\end{align*} 
%
\begin{equation}\label{eq:predictor1}
\quad= -\! \sum_{p = 1}^P a_p(\L_\Gr)\, \x_{t-p} \!+\! \sum_{q = 1}^Q b_q(\L_\Gr) \left(\x_{t-q|t-1} \!-\! \tilde{\x}_{t-q}\right).
\end{equation}
%
where in the last equality we used $\Exp[\eps_t] = \mathbf{0}_N$. We refer to $\tilde{\x}_{t}$ as the \emph{one-step ahead predictor}. The $k-$step ahead predictor can be obtained by repeating the above computation $k$ times.

The one-step ahead predictor for the GP-VAR model \eqref{eq.gcp_varma} can be obtained from \eqref{eq:predictor1} by setting $a_p(\L_\Gr) = \sum_{l = 0}^{L_p}\psi_{l,p}\L_\Gr^l$ for $p = 1, \ldots, P$ and $Q = 0$. In the sequel, we show that \eqref{eq:predictor1} yields the optimal decision from an MSE perspective.


%---------------------------------------------------------------------------------------------------
%---------------------------------------------------------------------------------------------------
\subsection{Mean Square Error Analysis}
\label{subsec_mse}

We now illustrate the impact of the predictor parameters $a_p(\L_\Gr)$ and $b_q(\L_\Gr)$ on the MSE of the one-step ahead predictor \eqref{eq:predictor1}.% and show that this corresponds to the smallest achievable MSE.

The main result is summarized in the following proposition.

\begin{proposition}
\label{prop:mse_1step}
Let $\x_t$ be the output of the joint causal model \eqref{eq:joint_causal_model} and let $a_p(\L_\Gr)$ and $b_q(\L_\Gr)$ be a given set of model parameters. Then, the MSE of the one-step ahead predictor \eqref{eq:predictor1} is
%
\begin{equation}
\label{eq:MSE1Step}
\text{MSE} =  \Exp\left[\|b_0(\L_\Gr)\eps_t\|_2^2		\right] = \trace\left(\bSigma_{\varepsilon}	\right),
\end{equation}
which corresponds to the smallest achievable MSE.
\end{proposition}

(The proof is given in the Appendix.)











==> journal revised/section_numres.tex <==
% !TEX root = main.tex

This section tests the proposed models in four different scenarios: the Molene weather data set, the NOAA U. S. temperature data set, a walking dog dynamic mesh, and a simulated susceptible-infected (SI) epidemic spreading over a flight network.
%

{The predictors in Section~\ref{subsec_jcmg} are compared with: $(i)$ the disjoint univariate ARMA that predicts each time series per node; $(ii)$ the standard VAR \cite{lutkepohl2005new}; $(iii)$ the RGP-VAR from \cite{mei2017signal}; $(iv)$ the LMS on graphs algorithm from \cite{di2016adaptive}; and $(v)$ the RLS on graphs algorithm from \cite{di2017adaptive}. For the LMS and RLS on graphs algorithms, we considered samples collected on all nodes. The tracking performance of the approach introduced in Section~\ref{sec.subset} is compared with the Wiener inpainting \cite{Perraudin2016} (applied at each time instant) and the kernel Kalman filter (KKF) \cite{romero2016kernel}. For the KKF, we considered subsampled measurements only at time $t$.}


\rev{For all models, we find the respective parameters by cross-validation, as discussed in \cite{friedman2001elements}.}
%
With reference to Fig.~\ref{fig.fit_proc}, the time series is split along the temporal dimension into two parts: the in-sample data and the out-of-sample (or testing) data.
%
The in-sample data are further split into a training and a validation set. The estimation procedure starts with first fitting each model with different model parameters (\eg different values for $P$ and $Q$ in the G-VARMA predictor) to the training data and measures their performance on the validation set. Then, the selected parameters are the one that yield the lowest root normalized MSE (rNMSE) defined as
%
\begin{equation}\label{eq.av_rNMSE}
\text{rNMSE} = \sqrt{\frac{\sum_{t = 1}^\tau\|\tilde{\boldsymbol{\theta}}_t - \boldsymbol{\theta}_t	\|_2^2}{\sum_{t = 1}^\tau\|\boldsymbol{\theta}_t	\|_2^2}},
\end{equation}
%
for some unknowns $\boldsymbol{\theta}_1, \ldots, \boldsymbol{\theta}_\tau$ and respective estimates $\tilde{\boldsymbol{\theta}}_1, \ldots, \tilde{\boldsymbol{\theta}}_\tau$. Finally, the model is refitted with the selected parameters to the entire in-sample data and tested on the out-of-sample data. 

We indicate with $\sigma_{\text{g}}$ the Gaussian width used to perform the spectral smoothing along the graph dimension [cf. \eqref{eq.spec_smooth}] and with $\gamma$ the regularization parameter that determines a bias-variance trade-off in finding the ARMA coefficients along the temporal dimension\footnote{This is a regularization parameter used by the Matlab function armax.m that penalizes the $\ell_2$ norm of the ARMA coefficients.} \cite{ljung1998system,wills2005gradient}. In the simulations, we made use of the GSP toolbox \cite{perraudin2014gspbox}.

%
\begin{figure}[t]
\centering
\includegraphics[width=.7\columnwidth]{figures/fit_process.png}
\caption{Model fitting process \cite{friedman2001elements}.}
\label{fig.fit_proc}
\end{figure}
%

%%%%%
\begin{figure*}[!t]
\centering
\begin{subfigure}[h]{0.255\linewidth}
\includegraphics[width=\linewidth,trim={1.5cm 1.5cm 1.2cm 1cm},clip]{figures/molene_map_1}
\caption{}
\end{subfigure}
\hfill
\begin{subfigure}[h]{0.33\linewidth}
\includegraphics[width=\linewidth,trim={0.85cm 0.35cm 0.85cm 0.35cm},clip]{figures/dog_t=31.pdf}
\caption{}
\end{subfigure}
\hfill
\begin{subfigure}[h]{0.33\linewidth}
\includegraphics[width=\linewidth,trim={.8cm 2cm .8cm 1cm},clip]{figures/e_Epid_graph_1}
\caption{}
\end{subfigure}%
\caption{Graph topologies for the considered scenarios. (a) Molene graph. The vertex in red is the one selected to illustrate the prediction performance. \rev{(b) Dog mesh graph. In building the graph, we considered unknown the manifold structure. Thus, we can see edges connecting nodes in different legs that are close by each-other (in the time step on which the graph was constructed).} (c) Airline connectivity graph. \rev{The nodes in blue are in susceptible (S) state, while the random picked node in red (Mumbai) is in the infected (I) state.}}
\label{fig.2Scen_graphs}
\end{figure*}

\subsection{Considered scenarios and data pre-processing}

In the following, we discuss the four datasets used in our evaluation and provide details for graph construction and preprocessing.

\vskip1mm
\noindent\textbf{Molene data set.} The Molene data set contains hourly temperature measurements of $N = 32$ weather stations near Brest (France) for $T = 744$ hours. We consider a geometric graph (illustrated in Fig.~\ref{fig.2Scen_graphs} (a)) \rev{built from the node coordinates using the default nearest neighbor approach of \cite{perraudin2014gspbox}. This graph follows a $10-$NN construction and the weight of the edge $(i,j)$ follows the Gaussian kernel 
%
\begin{equation*}
[\W_\Gr]_{ij} = \text{exp}\big(-\text{dist}(i,j)/\overline{\text{dist}}	\big)
\end{equation*}
%
where $\text{dist}(i,j)$ is the Euclidean distance between stations $i$ and $j$ and $\overline{\text{dist}}$ is the average Euclidean distance of all sensors.
}The red station is used later on to illustrate the temperature prediction.
%
The Laplacian matrix $\L_\Gr$ is normalized to have a unitary spectral norm. Before the fitting process, the in-sample mean is subtracted from the raw data.

\vskip1mm
\noindent\rev{\textbf{NOAA data set.} This is another temperature data set and comprises of hourly temperature recordings at $N = 109$ stations across the United States in 2010 \cite{nooaDataset} for a total of $T = 8759$ hours. This data set has been used by four graph-based alternative techniques that we compare with, respectively the RGP-VAR \cite{mei2017signal}, the LMS and RLS on graphs \cite{di2017adaptive}, and by the KKF \cite{romero2016kernel}. We use the same graph structure as \cite{di2017adaptive} and \cite{romero2016kernel}, which is built following the approach of \cite{mei2017signal} and relies on the $7-$NN geographical distances. The combinatorial Laplacian ${\L}_{\mathcal{G}}$ is used to represent the graph connectivity and the in-sample mean is subtracted from the raw data before preprocessing.
}
\vskip1mm
\noindent\textbf{Walking dog mesh.} We start from the 3D coordinates of a mesh depicting a walking dog~\cite{gall2009motion}. We aim at predicting the average point position along the three coordinates. The mesh has $N = 251$ points (nodes) over $T = 59$ time steps. \rev{The graph follows a $10$-NN construction built from the coordinates at $t = 1$ and is illustrated in Fig.~\ref{fig.2Scen_graphs} (b). This mesh is sparser than the one in  \cite{grassi2017time} (where this data set is used to remove noise) to reduce the computational time.} As a preprocessing step, we again subtract the in-sample mean from the data and, as normalization, we divide by the largest absolute value.

\vskip1mm
\noindent\textbf{SI epidemic diffusion.} This scenario considers an epidemic diffusion following the susceptible-infected model \cite{nowzari2016analysis} over $N = 100$ international airports. The graph, depicted in Fig.~\ref{fig.2Scen_graphs} (c), captures the airline connections with edge weights $[\W_\Gr]_{i,j} = [\W_\Gr]_{j,i} = 1$ if there is a flight connection between two airports and zero otherwise. The graph has $3565$ edges and an average degree of $35.4$. $\L_\Gr$ is normalized to have a unitary spectral norm and the in-sample mean is subtracted from the data.

The time-varying process of interest is the daily evolution of the infection chance of each node (airport). We select an infection rate of $10^{-3}$ and consider a small fixed population occupying each airport (60 targets). %A more involved model would instead consider variable population sizes selected according to historical data of airport occupancy. 
The infected targets are assumed to return to the susceptible state after 12 days and the overall epidemic diffusion is analyzed for $T = 122$ days. \rev{In the initial state, all targets at the blue nodes are in the susceptible-state (S-state), while all targets at the red node are in the infected-state (I-state).}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
\centering
\fbox{\begin{minipage}{\textwidth}%
    \begin{subfigure}{.5\columnwidth}
\centering
\includegraphics[width=\columnwidth,trim={.3cm 0 .7cm 0},clip]{figures/e_rNMSE_steps_molene_new.pdf}
\caption{rNMSE versus the prediction steps for the different methods. The used parameters are: [G-VARMA \eqref{eq:joint_causal_model} : $P = 3$, $Q = 0$, $\sigma_{\text{g}} = 0$, $\gamma = 0$], [GP-VAR: $P = 2$, $L_p = L = 4$, $\sigma_{\text{g}} = 0$], [ARMA: $P = 4$, $Q = 0$, $\gamma = 0$], [VAR \cite{lutkepohl2005new}: $P = 2$], [RGP-VAR \cite{mei2017signal}: $P = 3$], [LMS on Graphs  \cite{di2016adaptive}: B.width $= 16$, $\mu_{\text{LMS}} = 1.2$], [RLS on Graphs \cite{di2017adaptive}: B.width $=16$, $\beta_{\text{RLS}} = 0.05$].}
\label{fig.mol_pred_pow}
    \end{subfigure}
\hfil
    \begin{subfigure}{.4\columnwidth}
\centering
\includegraphics[width=\columnwidth,trim={.55cm 0 .7cm .35cm},clip]{figures/e_Molene_predVal13_new.pdf}\vskip-2mm
\caption{True temperature in degrees Celsius and the G-VARMA one- and three-steps ahead predictions at the red sensor in Fig.~\ref{fig.2Scen_graphs} (a).}
\label{fig.mol_true_sig}
    \end{subfigure}\\
\vskip2.5mm
    \begin{subfigure}{.5\columnwidth}
    \centering
\includegraphics[width=\columnwidth,trim={.3cm 0 .7cm 0},clip]{figures/noaas_steps.pdf}
\caption{rNMSE versus the prediction steps for the different methods. The used parameters are: [G-VARMA \eqref{eq:joint_causal_model} : $P = 3$, $Q = 0$, $\sigma_{\text{g}} = 0$, $\gamma = 0$], [GP-VAR: $P = 3$, $L_p = L = 3$, $\sigma_{\text{g}} = 0$], [ARMA: $P = 3$, $Q = 0$, $\gamma = 0$], [RGP-VAR \cite{mei2017signal}: $P = 2$], [LMS on Graphs  \cite{di2016adaptive}: B.width $= 40$, $\mu_{\text{LMS}} = 1.5$], [RLS on Graphs \cite{di2017adaptive}: B.width $=40$, $\beta_{\text{RLS}} = 0.5$]. A zoomed in version of one one-step ahead prediction is provided in Fig.~\ref{fig.noaaZoom} in the Appendix.}
\label{fig.noaa_pred_pow}
    \end{subfigure}
\hfil
    \begin{subfigure}{.4\columnwidth}
\centering
\includegraphics[width=\columnwidth,trim={.45cm 0 .7cm .35cm},clip]{figures/noaas_pred13.pdf}\vskip-2mm
\caption{True temperature in degrees Fahrenheit and the G-VARMA one- and three-steps ahead predictions for the same node visualized \cite{di2017adaptive}.}
\label{fig.noa_true_sig}
    \end{subfigure}
    \end{minipage}}
    \caption{Comparison of the predictive power of the different algorithms in the weather datasets. (a)-(b) Molene data set. (c)-(d) NOAA data set. The results in plots (b) and (d) are w.r.t. the out-of-sample data.}
    \label{fig.motherPred}
    \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure*}[!t]
\centering
\fbox{\begin{minipage}{\textwidth}%
    \vskip2.5mm
    \begin{subfigure}{.5\columnwidth}
    \centering
\includegraphics[width=\columnwidth,trim={.3cm 0 .7cm 0},clip]{figures/e_rNMSE_steps_dog_new.pdf}
\caption{rNMSE versus the prediction steps for the different methods. The used parameters are: [G-VARMA \eqref{eq:joint_causal_model} : $P = 3$, $Q = 0$, $\sigma_{\text{g}} = 0$, $\gamma = 0$], [GP-VAR: $P = 4$, $L_p = L = 3$, $\sigma_{\text{g}} = 0.25$], [ARMA: $P = 2$, $Q = 0$, $\gamma = 0$], [RGP-VAR \cite{mei2017signal}: $P = 3$], [LMS on Graphs  \cite{di2016adaptive}: B.width $= 16$, $\mu_{\text{LMS}} = 1.35$], [RLS on Graphs \cite{di2017adaptive}: B.width $=16$, $\beta_{\text{RLS}} = 0.05$].}
\label{fig.dog_pred_pow}
    \end{subfigure}
\hfil
    \begin{subfigure}{.4\columnwidth}
\centering
\includegraphics[width=\columnwidth,trim={.45cm 0 .7cm .35cm},clip]{figures/e_Dog_predVal13_new.pdf}\vskip-2mm
\caption{True x-axis value and the G-VARMA one- and three-steps ahead predictions at the the node that has the largest variability in the true signal.}
\label{fig.dog_true_sig}
    \end{subfigure}\\
\vskip2.5mm
    \begin{subfigure}{.5\columnwidth}
\centering
\includegraphics[width=\columnwidth,trim={.3cm 0 .7cm 0},clip]{figures/e_rNMSE_steps_epid_new.pdf}
\caption{rNMSE versus the prediction steps for the different methods. The used parameters are: [G-VARMA \eqref{eq:joint_causal_model} : $P = 4$, $Q = 0$, $\sigma_{\text{g}} = 0$, $\gamma = 0$], [GP-VAR: $P = 2$, $L_p = L = 5$, $\sigma_{\text{g}} = 0$], [ARMA: $P = 4$, $Q = 0$, $\gamma = 0$], [RGP-VAR \cite{mei2017signal}: $P = 2$], [LMS on Graphs  \cite{di2016adaptive}: B.width $= 16$, $\mu_{\text{LMS}} = 1.3$], [RLS on Graphs \cite{di2017adaptive}: B.width $=16$, $\beta_{\text{RLS}} = 0.05$].}
\label{fig.epid_pred_pow}
    \end{subfigure}
\hfil
    \begin{subfigure}{.38\columnwidth}
\centering
\includegraphics[width=\columnwidth,trim={.45cm 0 .7cm .35cm},clip]{figures/e_Epid_predVal13_new.pdf}\vskip-2mm
\caption{Evolution of the infection portion on the whole graph and the G-VARMA one- and three-step ahead predictions.}
\label{fig.epid_true_sig}
    \end{subfigure}
    \end{minipage}}
    \caption{Comparison of the predictive power of the different algorithms in the three scenarios. (a)-(b) Walking dog mesh. (c)-(d) SI epidemic diffusion. The results in plots (b) and (d) are w.r.t. the out-of-sample data.}
    \label{fig.motherDogSI}
    \end{figure*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%
\begin{figure*}[t]
\centering
\begin{subfigure}[h]{0.24\linewidth}
\hskip2mm\includegraphics[width=\linewidth,trim={1cm 0.5cm 1.0cm 0cm},clip]{figures/dog_t=31_withGT.pdf}
%\caption{}
\end{subfigure}
\begin{subfigure}[h]{0.24\linewidth}
\hskip2mm\includegraphics[width=\linewidth,trim={1cm 0.5cm 1.0cm 0cm},clip]{figures/dog_t=33_withGT.pdf}
%\caption{}
\end{subfigure}
%\hfill
\begin{subfigure}[h]{0.24\linewidth}
\hskip2mm\includegraphics[width=\linewidth,trim={1cm 0.5cm 1.0cm 0cm},clip]{figures/dog_t=35_withGT.pdf}
%\caption{}
\end{subfigure}
\begin{subfigure}[h]{0.24\linewidth}
\hskip2mm\includegraphics[width=\linewidth,trim={1cm 0.5cm 1.0cm 0cm},clip]{figures/dog_t=37_withGT.pdf}
%\caption{}
\end{subfigure}
\caption{\rev{Four test time steps of the three step ahead G-VARMA prediction in the walking dog experiment. The red points correspond to the prediction and the black to the ground-truth. The four time steps are causal with a delay of 2 steps.}}
\label{fig.dogPos}
\end{figure*}
%%%%%


\subsection{Prediction performance} \label{subsec:predPerf}
We first compare the predictive power of the different algorithms. \rev{For all scenarios, the training, cross-validation, and test data consist respectively of $35\%$, $15\%$, and $50\%$.} The parameter fitting criterion is the average of the rNMSE \eqref{eq.av_rNMSE} over the five-step ahead prediction. \rev{The results for the weather data sets (Molene and NOAA) are shown in Fig.~\ref{fig.motherPred}, while those of the waling dog and epidemic diffusion in Fig.~\ref{fig.motherDogSI}.}

\vskip1mm
\noindent\textbf{Molene data set.} Fig.~\ref{fig.mol_pred_pow} shows the prediction rNMSE up to five future steps (hours) for all methods. We see that the proposed G-VARMA and GP-VAR models achieve the best performance over other approaches, although the error is small only for predictions of up to three hours. The GP-VAR falls sightly behind the G-VARMA in terms of accuracy due its more constrained form (localized graph filters).

Fig.~\ref{fig.mol_true_sig} depicts the true out-of-sample signal and the one and three-steps ahead prediction of the G-VARMA model at the red sensor in Fig.~\ref{fig.2Scen_graphs} (a). We see that the one-step ahead prediction matches well the true signal with a deviation lower than 0.5 degrees, while the three-steps ahead prediction is characterized by a larger deviation (up to $3$ degrees Celsius).

\vskip1mm
\noindent\rev{\textbf{NOAA data set.} Fig.~\ref{fig.noaa_pred_pow} shows the prediction power of the different algorithms in this scenario. We first remark that the training of standard VAR crashed continuously due to the high number of parameters involved. The graph-based techniques on the other hand, lead to trainable models due to the reduced number of parameters. These results show that the proposed methods exploit better the graph parameterization and yield the minimum performance. 
}

\rev{The disjoint ARMA compares well with the proposed algorithms and yields values closer to minimum achieved by the G-VARMA. This is not entirely surprising for two main reasons. First, the time series present a strong temporal stationarity which is known to be well exploited by ARMA models. Second, we fixed the graph as in \cite{di2017adaptive} and \cite{romero2016kernel} for a direct comparison with these methods. This choice penalizes the stationarity assumptions. Therefore, we believe that the performance of the G-VARMA and the GP-VAR can be further improved by optimizing the graph topology.
}

\rev{As a final remark, note that we used the parameters of the LMS ($\mu_{\text{LMS}} = 1.5$) and RLS ($\beta_{\text{RLS}} = 0.5$) on graphs algorithms as fixed\footnote{\rev{This is done to ensure a fair comparison with these methods.}} by \cite{di2017adaptive}. By cross-validation, we found that the optimal values are $\mu_{\text{LMS}} = 1.75$ and $\beta_{\text{RLS}} = 0.05$. These cross-validated values lead to a slightly lower rNMSE, but still significantly worse when compared with the proposed methods and to the disjoint ARMA.}

\rev{Fig.~\ref{fig.noa_true_sig} shows the one- and the three-steps ahead predictions at node $25$, which is the same used to display the tracking results of LMS, RLS, and KKF in \cite{di2017adaptive}. We observe that the one-step ahead prediction matches relatively well the true signal value, while a bigger error is observed for the three-step ahead prediction especially closer to the transition points.}

\vskip1mm
\noindent\textbf{Walking dog mesh.} The rNMSE vs number of step ahead results are shown in Fig.~\ref{fig.dog_pred_pow}. The classic multivariate VAR is not shown as it yielded unstable predictions (as the number of time series is large). Incorporating the graph in the predictive models seems to avoid these issues. In fact, all graph-based approaches give more stable predictors. Additionally, the RGP-VAR \cite{mei2017signal} yields the worst prediction due to fewer DoF. A comparison with its generalized version, i.e., the GP-VAR, shows an rNMSE close to the best performance. We note that the rNMSE gap between the proposed methods and other graph-based alternatives is larger w.r.t. the Molene data set. The spectral smoothing plays a role here for the GP-VAR since the signal evolution (i.e., the point position) is more regular along the graph dimension than temperature. This is reflected in a higher value of $\sigma_g$.

Fig.~\ref{fig.dog_true_sig} illustrates the true signal evolution along with its G-VARMA  one- and three-step ahead predictions. The selected node is the one that presents the largest peak-to-peak variability in the true signal. Compared to the Molene data set, we note a worse three-step ahead prediction, while the one-step ahead prediction is still comparable. \rev{Fig.~\ref{fig.dogPos} further shows the true dog position in four causal time steps and the three step ahead G-VARMA prediction. We can observe that the proposed model matches well the dog position in most of the nodes. Larger errors are observed around the body parts that move the most, e.g., legs and tail.}


\vskip1mm
\noindent\textbf{SI epidemic diffusion.} The results for this scenario are shown in Figs.~\ref{fig.epid_pred_pow}-\ref{fig.epid_true_sig}. Similarly to the walking dog mesh, the VAR model yields unstable results. From the results in Fig.~\ref{fig.epid_pred_pow}, all graph-based methods offer a similar rNMSE for the one-step ahead prediction\footnote{An exception is the RGP-VAR recursion \cite{mei2017signal}, which offers a worse performance. However, the focus of this approach is to learn a topology that facilitates prediction and it might suffer when the fixed graph structure differs from the learned one.}. The latter highlights the importance of the underlying topology in building prediction models, since the univariate ARMA yields a larger rNMSE than the proposed models. For more than one-step ahead predictions, we see that the proposed approaches exploit better the graph and keep yielding a smaller rNMSE than the adaptive algorithms. \rev{Nevertheless, starting from three-steps ahead, the univariate ARMA offers a similar rNMSE as the proposed methods.}

We make the subsequent remarks. First, the rNMSE is higher in this data set w.r.t. the previous two cases. We attribute this degradation to the abrupt transitions in the patient recovery instances (i.e., every $12$ days). Second, also in this data set we see that the G-VARMA does not have coefficients in the MA part. {We have found that the value of $Q$ varies depending on the amount of training data and cross-validation criterion.} For instance, the G-VARMA model with $P = 1$, $Q = 1$, $\sigma_g = 0.5$, and $\gamma = 0.44$ yields a better performance in the test data than the one shown in Fig.~\ref{fig.epid_pred_pow}, though in the cross-validation data its performance is suboptimal.
%
%
%This behavior is transcendent from the used amount of in-sample and training data. 
%In fact, even for the other two scenarios, we have achieved full G-VARMA recursions with a different percentage of training samples. 
Finally, we have observed that the chosen models are characterized by a bounded memory in time. That is, only a few past realizations are useful for the prediction task. The GP-VAR model shows that there is a larger graph influence (i.e., information from further nodes) in the model. Indeed, information from nodes up to four hops away is exploited in Fig.~\ref{fig.epid_pred_pow} and in Fig.~\ref{fig.mol_pred_pow}.

To conclude, Fig.~\ref{fig.epid_true_sig} illustrates the evolution of the I-state on the whole graph and the respective G-VARMA predictions. The proposed model follows relatively well the I-state evolution for one-step ahead prediction with an error up to $4\%$, yet its performance degrades in the three-step ahead prediction\footnote{This may be improved by using other model parameters.}. {The decreased amplitude (w.r.t the ground truth) is mainly attributed to a couple outlier nodes where the I-state evolution is not predicted correctly, and, therefore, influence the overall result.}

%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth,trim={.3cm 0 .7cm 0},clip]{figures/e_molene_inSampleData2_new.pdf}
\caption{One-step ahead prediction rNMSE versus the percentage of in-sample-data for the different algorithms in the Molene data set. The RLS on graphs \cite{di2017adaptive} is not shown here and offers a similar performance as the LMS on graphs algorithm. Note that the standard VAR could not be trained for $10\%$ in-sample data.}\vskip-.2cm
\label{fig.mol_insample}
\end{figure}
%%%%%%%%%%%%%%

\subsection{In-sample data effect}

We now analyze the effect of the in-sample data size on prediction accuracy. For consistency with the earlier results, {we kept the cross-validation data to be $30\%$ of the in-sample data,} whereas the model parameters are selected to minimize the one-step ahead rNMSE.

Fig.~\ref{fig.mol_insample} shows the one-step ahead prediction rNMSE as a function of the in-sample data percentage for the Molene data set. We first highlight that the multivariate VAR \cite{lutkepohl2005new} is the one that suffers the most in low in-sample data regimes. For this model, we see a clear trend of rNMSE reduction when more data are used for estimating the coefficients. All graph-based methods are more robust to low in-sample data sizes since they have fewer parameters. The latter along with the spectral smoothing seems to play a role when the amount of training data is limited. The slight variation in the rNMSE for more training data is within the experimental variance. When the percentage of in-sample data is very small ($10\%$), the GP-VAR improves upon G-VARMA due to its fewer DoF.

We conclude that the proposed methods make a better use of the underlying topology and provide a good trade-off between the model complexity and the amount of training data.
%
As a final remark, we do not show these results for the other scenarios since the VAR \cite{lutkepohl2005new} recursion (which is the one to compare with) does not lead to stable predictors.

%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=.9\columnwidth,trim={.3cm 0 .7cm 0},clip]{figures/lowRank4Datasets}
\caption{Gained speed-up versus the loss in prediction rNMSE for the G-VARMA model estimated using the low-rank representation of the process. \rev{Both axes are in log scale to improve the visibility. For the NOAA data set, the maximum rNMSE loos is $0.13$ with a speed-up of $16$.}}
\label{fig.mol_lowRank}
\end{figure}
%%%%%%%%%%%%

\subsection{Low-rank model effect}
\label{subsec_lowRank}

We now test the effects of the low-rank G-VARMA coefficient estimation described in Theorem~\ref{theo.low_rank}. Under the settings of Fig.~\ref{fig.motherPred}, we estimate the models by ignoring different portions of the process JPSD. We considered nine ignoring percentages log-spaced in the interval $[0.74\%, 5\%]$ and evaluate the rNMSE loss and the code speed-up. The code running time is averaged over $100$ iterations and the speed-up achieved using the low-rank procedure is compared w.r.t. the case where the entire JPSD is used.

Fig.~\ref{fig.mol_lowRank} shows the gained speed-up as a function of the rNMSE degradation in the one-step ahead prediction. Each marker corresponds to an increasing data ignorance percentage. The obtained results show a trade-off between prediction accuracy and computational time. We see that the most sensitive scenario to data ignorance is the NOAA data set as its NMSE loss increases the fastest, while the least sensitive scenario is the SI epidemic one. This much higher sensitivity of the NOAA data set is due to the misalignment between the used graph and the stationarity assumptions. Better results are expected in this data set with a topology that imposes a stronger joint stationarity. These observations highlight, nevertheless, the sparsity in the process JPSD which can be exploited to ease the model estimation costs.



%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth,trim={.3cm 0 .4cm 0},clip]{figures/e_MSE_track_new}
\caption{rNMSE versus the cardinality of sampling set for different tracking algorithms in the Molene data set. The used parameters are: [G-VARMA \eqref{eq:joint_causal_model} : $P = 3$, $Q = 0$, $\sigma_{\text{g}} = 0$, $\gamma = 0$], [Wiener inpainting, $\w_t \sim \mathcal{N}(\mathbf{0}_N, 0.5\I_N)$], [KKF \cite{romero2016kernel}: $\mu_{\text{KKF}} = 10^{-7}$, $\sigma_{\text{KKF}} = 1.25$, $b_{\text{KKF}} = 0.09$].}
\label{fig.mol_track}
\end{figure}
%%%%%%%%%%%%%%


\subsection{Tracking performance}

We here evaluate the tracking performance of the G-VARMA model on the Molene and NOAA data sets. The G-VARMA parameters are the same as the one used in Section~\ref{subsec:predPerf} with coefficients estimated following the low-rank model and ignoring $1.5 \%$ of the process JPSD. The noise power for the Wiener inpainting is cross-validated following the procedure in Fig.~\ref{fig.fit_proc} using all the $50\%$ in-sample data. \rev{For the KKF, we cross-validated the different parameters, i.e., the KKF kernel weight ($\mu_{\text{KKF}}$), the diffusion coefficient ($\sigma_{\text{KKF}}$), and the edge propagation weight ($b_{\text{KKF}}$) using all the $50\%$ in-sample data in the Molene data set. Instead, for the NOAA data set we used the parameters proposed in \cite{romero2016kernel}.} During the training process, $75\%$ of the nodes are sampled uniformly at random and the considered score is the tracking rNMSE. To the G-VARMA tracker, a small artificial noise is added to the out-of-sample data to avoid numerical issues when inverting $\H_t$. In the test phase, we average the rNMSE over $100$ random node selections and consider $\bar{\Scal}_t = \Vx$.

\vskip1mm
\textbf{Molene data set}. Fig.~\ref{fig.mol_track} depicts the average tracking rNMSE as a function of the size $|\Scal_t|$ of the observation set. The proposed method is seen to improve substantially the accuracy of the G-VARMA predictor and outperforms the other approaches even with $N/4 = 8$ collected samples at time $t$. Wiener inpainting provides suboptimal predictions as it does not exploit the historical data. These results show also the benefits of the G-VARMA predictors over the Wiener inpainting and the KKF approach.

\vskip1mm
\rev{
\textbf{NOAA data set}. The tracking results for the NOAA data set are shown in Fig. \ref{fig.noaa_track}. The latter enforces the behavior of the different methods observed for the Molene data set. The Wiener inpainting still offers the worse performance as it does not explore the temporal dimension. Similarly, both the G-VARMA prediction and tracking offer a lower rNMSE than the KKF \cite{romero2016kernel}. The performance of the KKF can be slightly improved by using cross-validation (validated parameters $\mu_{\text{KKF}} = 10^{-6}$, $\sigma_{\text{KKF}} = 1.5$, $b_{\text{KKF}} = 0.15$).}

\rev{In Fig. \ref{fig.noaaTrackZoom} (see the Appendix), we zoomed in the performance of the proposed G-VARMA tracking methods. A larger cardinality of the sampling set leads to small reduction of the rNMSE. We mainly attribute this minimal improvement to the mismatch between the data behavior and the G-VARMA model. Further reduction of the rNMSE can be obtained by selecting the $|\mathcal{S}_t|$ in a sparse sensing fashion \cite{chepuri2016sparse} and by introducing seasonality into the G-VARMA model \cite{brockwell2002introduction}.}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\centering
    \begin{subfigure}{\columnwidth}
\centering
\includegraphics[width=\columnwidth,trim={.3cm 0 .4cm 0},clip]{figures/UStemp_track}
\caption{Comparison of the different methods.}
\label{fig.noaa_track}
    \end{subfigure}
    \caption{rNMSE versus the cardinality of sampling set for different tracking algorithms in the Molene data set. The used parameters are: [G-VARMA \eqref{eq:joint_causal_model} : $P = 3$, $Q = 0$, $\sigma_{\text{g}} = 0$, $\gamma = 0$], [Wiener inpainting, $\w_t \sim \mathcal{N}(\mathbf{0}_N, 0.5\I_N)$], [KKF \cite{romero2016kernel}: $\mu_{\text{KKF}} = 10^{-7}$, $\sigma_{\text{KKF}} = 1.8$, $b_{\text{KKF}} = 0.01$]. A zoomed in version of the G-VARMA tracking algorithm is provided in the Appendix.}
    \label{fig.motherTracNoaa}
    \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%







%\vskip 1mm
%\noindent\textbf{Subset forecasting.} In this final scenario, we evaluate the performance of the CG-VARMA model when measurements at time $t$ are collected from a subset of nodes [cf. Section~\ref{sec.subset}]. We considered the in-sample data to be $50\%$ of the total measurements and we focus on the one-step-ahead prediction. 
%
%In this comparison, the multivariate VAR model is not included since we did not find a stable implementation for it. We attribute these numerical instabilities to the high spatial data dimension. Similar degradation performance are commonly observed in VAR and VARMA models when the temporal dimension of the time series is not much larger than the number of time series. 

%\subsection{Results on the Molene weather data set}\label{sec.molen_exp}
%The Molene data set contains hourly temperature measurements of $N = 32$ weather stations in the region of Brest (France) for $T = 744$ hours. The used graph is a geometric graph constructed from the node coordinates using the default $k$NN approach of \cite{perraudin2014gspbox} illustrated in Fig.~\ref{fig.molene_graph}. The graph Laplacian is normalized to have a unitary spectral norm. Before fitting the different models, we pre-processed the raw data by subtracting first the empirical in-sample mean.
%
%\vskip 1mm
%\noindent\textbf{Prediction power.} %We start our analysis by evaluating the predictive power of our algorithms up to five future steps. %The in-sample data consists of the first $50\%$ of the temperature measurement, out of which $95\%$ are training data and $5\%$ cross-validation data. The different algorithm parameters are found following the procedure in Fig.~\ref{fig.fit_proc} with selection criterion the average root normalized MSE (rNMSE) over the five steps ahead predictions.
%%The training and validation data consist respectively of $35\%$ and $15\%$ of the entire dataset and the parameter fitting criterion is the average rNMSE over the five steps ahead prediction. 
%
%%\begin{figure}[t]
%%\centering
%%\includegraphics[width=\columnwidth,trim={.3cm 0 .7cm 0},clip]{figures/e_Molene_predpow1.pdf}
%%\caption{rNMSE versus the prediction steps for the different methods. The used parameters are: [G-VARMA \eqref{eq:joint_causal_model} : $P = 4$, $Q = 0$, $\sigma_{\text{s}} = 0.125$ \elvin{There should be another parameter here, right?}], [GP-VAR: $P = 2$, $L_p = L = 4$, $\sigma_{\text{s}} = 0.125$], [ARMA: $P = 1$, $Q = 0$], [VAR \cite{lutkepohl2005new}: $P = 1$], [RGP-VAR \cite{mei2017signal}: $P = 4$], [LMS on Graphs  \cite{di2016adaptive}: B.width $= 16$, $\mu_{\text{LMS}} = 1.2$], [RLS on Graphs \cite{di2017adaptive}: B.width $=16$, $\beta_{\text{RLS}} = 0.05$].}
%%\label{fig.mol_pred_pow}
%%\end{figure}
%
%Fig.~\ref{fig.mol_pred_pow} shows the prediction rNMSE up to five future steps for all methods. We observe that the proposed G-VARMA and GP-VAR models achieve the best performance over their contenders, though the prediction error is reasonable up to two steps in the future. Moreover, we note that the GP-VAR model looses in performance w.r.t. the G-VARMA in predicting more than three steps ahead.

%We note that the proposed CG-VARMA and CGP-VAR models achieve the best performance over their contenders, though the prediction error is reasonable up to two steps in the future. Moreover, we observe that the CGP-VAR looses in performance in predicting five steps ahead.
%
%%\begin{figure*}[t]
%%\centering
%\begin {table*}[t]
%\caption {Parameters in the Molene data set. N/A $\equiv$ not applicable.\textcolor{red}{I'm leaving the table for now, we can put the parameters in the legend.}} \label{tab:moleneParam} 
%\begin{center}
%\begin{tabular}{|l||*{8}{c|}}\hline
%\backslashbox{Model}{Parameter}
%&\makebox[1.5em]{P}&\makebox[1.5em]{Q}&\makebox[3em]{Lp = L}
%&\makebox[3em]{B.width}&\makebox[2em]{$\mu_{\text{LMS}}$}&\makebox[2em]{$\beta_{\text{RLS}}$}&\makebox[8em]{Estimation Time (s)}\\\hline\hline
%CG-VARMA &2&1&N/A&N/A&N/A&N/A&5.4\\\hline
%CGP-VAR &2&N/A&3&N/A&N/A&N/A&0.9\\\hline
%ARMA &5&1&N/A&N/A&N/A&N/A&8.4\\\hline
%VAR &&&&&\\\hline
%RCGP-VAR &2&N/A&N/A&N/A&N/A&N/A&2.1\\\hline
%LMS &N/A&N/A&N/A&16&1.2&N/A&0.1\\\hline
%RLS &N/A&N/A&N/A&16&N/A&0.05&1.2\\\hline
%\end{tabular}
%\end{center}
%\end {table*}
%%\end{figure*}

%\begin{figure}[t]
%\centering
%\includegraphics[width=\columnwidth,trim={.4cm 0 .7cm .35cm},clip]{figures/e_Molene_predVal13.pdf}
%\caption{True temperature in degrees Celsius and the G-VARMA one and three steps ahead predictions at the red sensor in Fig.~\ref{fig.molene_graph}.}
%\label{fig.mol_true_sig}
%\end{figure}

%To provide a more physical interpretation to the above rNMSEs, in Fig.~\ref{fig.mol_true_sig} we depict the true out-of-sample signal and the one and three steps ahead prediction of the G-VARMA model at the red sensor in Fig.~\ref{fig.molene_graph}. We observe that the one-step-ahead prediction matches well the true signal with a deviation of at most 0.5 degrees, while the three steps ahead prediction is characterized by a larger deviation (up to $3$ degrees Celsius).

%\vskip 1mm
%\noindent\textbf{In-sample data effect.}% This second scenario analyzes the effects of the in-sample data on the prediction power of the different algorithms. As in the previous scenario, we considered the cross-validation data to be $5\%$ of all the in-sample data. In this instance, the different method parameters are chosen as the one that yield the minimum one-step-ahead rNMSE.

%Fig.~\ref{fig.mol_insample} shows the rNMSE of the one-step-ahead prediction as a function of the percentage of in-sample data\footnote{Observe that for the $50\%$ in-sample data the results in Fig.~\ref{fig.mol_insample} are different from those in Fig.~\ref{fig.mol_pred_pow} due to the different criterion for selecting the parameters.}. We first observe that the rNMSE does not reduce monotonically when more in-sample data are considered. The latter suggests that even $10\%$ of the data can be enough for the different algorithms due to their low orders. Additionally, we remark that the proposed CG-VARMA and CGP-VAR algorithms do outperform their contenders with the latter offering the lowest rNMSE.

%\vskip 1mm
%\noindent\textbf{Low-rank effect.} \textcolor{red}{to do.}


%\vskip 1mm
%\noindent\textbf{Subset forecasting.} In this final scenario, we evaluate the performance of the CG-VARMA model when measurements at time $t$ are collected from a subset of nodes [cf. Section~\ref{sec.subset}]. We considered the in-sample data to be $50\%$ of the total measurements and we focus on the one-step-ahead prediction. 
%
%
%
%%\subsection{Results on the walking dog mesh}
%%In this second scenario, we consider a 3D walking dog mesh and aim predicting the future position. The mesh consists of $N = 251$ points (nodes) over $T = 59$ timestamps. The graph consists of a 10-nearest neighbor graph built from the coordinates in the first timestamp. The signal of interest is temporal evolution of the x-axis coordinate of each node. The data preprocessing consists of first removing the empirical mean along the dimension of interest and then normalizing the values by their maximum absolute value in each dimension.
%
%
%%\vskip 1mm
%%\noindent\textbf{Prediction power.} %We first evaluate the prediction power of the different algorithms up to 5 future steps under the same settings of the Molene data set. 
%In this comparison, the multivariate VAR model is not included since we did not find a stable implementation for it. We attribute these numerical instabilities to the high spatial data dimension. Similar degradation performance are commonly observed in VAR and VARMA models when the temporal dimension of the time series is not much larger than the number of time series.

%\begin{figure}[t]
%\centering
%\includegraphics[width=\columnwidth,trim={.3cm 0 .7cm 0},clip]{figures/e_Dog_predpow1.pdf}
%\caption{rNMSE versus the prediction steps for the different methods. The used parameters are: [G-VARMA \eqref{eq:joint_causal_model} : $P = 4$, $Q = 0$, $\sigma_{\text{s}} = 0.5$ \elvin{There should be another parameter here, right?}], [GP-VAR: $P = 4$, $L_p = L = 2$, $\sigma_{\text{s}} = 0.25$], [ARMA: $P = 2$, $Q = 0$], [RGP-VAR \cite{mei2017signal}: $P = 3$], [LMS on Graphs  \cite{di2016adaptive}: B.width $= 16$, $\mu_{\text{LMS}} = 1.35$], [RLS on Graphs \cite{di2017adaptive}: B.width $=16$, $\beta_{\text{RLS}} = 0.05$].}
%\label{fig.dog_pred_pow}
%\end{figure}


%Fig.~\ref{fig.dog_pred_pow} depicts the prediction rNMSE as a function of the prediction steps for the remaining methods. We first observe that the RGP-VAR \cite{mei2017signal} also yields bad prediction due to its limited degrees of freedom. Indeed, by observing the performance of its generalized version, i.e., the GP-VAR model, the rNMSE is close to the best performance. Additionally, we note that the performance gap between proposed methods and the other alternatives is bigger w.r.t. the Molene data set. We finally remark that the spectral smoothness parameters play a bigger role here, since the signal evolution (i.e., the node x-axis coordinate) is more regular along the graph dimension than the temperature variations.
%
%\begin{figure}[t]
%\centering
%\includegraphics[width=\columnwidth,trim={.4cm 0 .7cm .35cm},clip]{figures/e_dog_predVal13.pdf}
%\caption{True x-axis value and the G-VARMA one and three steps ahead predictions at the the node that has the largest variability in the true signal.}
%\label{fig.dog_true_sig}
%\end{figure}

%Finally, Fig.~\ref{fig.dog_true_sig} illustrates the true signal evolution along with its G-VARMA  one and three steps ahead predictions. The selected node is the one that presents the largest variability peak-to-peak in the true signal. With respect to the Molene data set, we observe a worse three steps ahead prediction, while the one-step-ahead prediction is still reasonable. 

%\vskip 1mm
%\noindent\textbf{In-sample data effect.}

%\textcolor{red}{Only prediction power, value tracking and training data effect. No low-rank and subsampling.}

%\subsection{Results on the SI epidemic diffusion model}

%\begin{figure}[t]
%\centering
%\includegraphics[width=.65\columnwidth,trim={2cm 2cm 1.5cm 1cm},clip]{figures/e_Epid_graph}
%\caption{Considered airline connectivity graph. The nodes in blue are in the S-state, while the random picked node in red (Mumbai) is in the I-state.}
%\label{fig.epid_graph}
%\end{figure}


%This third scenario simulates an epidemic diffusion following the standard susceptible-infected (SI) model \cite{} over the $N = 100$ major cities of Europe. \elvin{From the coordinates it is not Europe but world wide. We just pick the first 100, but are they sorted in the file? Do you have a reference for this?} The graph, depicted in Fig.~\ref{fig.epid_graph}, consists of the airline connections between these cities with edge weight $[\W_\Gr]_{i,j} = [\W_\Gr]_{j,i} = 1$ if there is a flight connection between the two cities and zero otherwise. The graph results in $3565$ edges and an average of $35.4$ connections per node.  Similarly to the Molene data set scenario, we again consider $\L_\Gr$ to have a unitary spectral norm and subtract the empirical mean from the data.

%The time-varying process of interest is the daily evolution of the infected portion of population in each node. Specifically, we considered a population of 60 targets in each airport and an infection rate of $10^{-3}$. The infected targets are assumed to naturally return to the susceptible state after a period of 12 days and the overall epidemic diffusion is analyzed for $T = 122$ days. In the initial network state, all targets at the blue nodes are in the S-state, while all targets at the red node are in the I-state.

%In the sequel, we again analyze the prediction rNMSE of the different algorithms and illustrate the prediction evolution at the initial seeding node.

%\vskip 1mm
%\noindent\textbf{Prediction power.} %The prediction rNMSE as a function of the future prediciton steps is shown in Fig.~\ref{fig.epid_pred_pow}. The model validation settings are similar to the previous two datasets. Here, we observe that the graph-based methods offer a similar prediction rNMSE for one-step-ahead prediction\footnote{An exception is the RGP-VAR model \cite{mei2017signal}, which offers a worse performance. However, we remark that the focus of this model is to learn a topology that facilitates prediction and it might suffer when the graph structure is fixed.}. The latter highlights the importance of the underlying topology in building prediction models, since the singular ARMA approaches per node yield a larger rNMSE. For more that one-step-ahead predictions, we see that the proposed approaches exploit better the graph structure and yield smaller rNMSE than the adaptive approaches.

%\begin{figure}[t]
%\centering
%\includegraphics[width=\columnwidth,trim={.3cm 0 .7cm 0},clip]{figures/e_Epid_predpow1.pdf}
%\caption{rNMSE versus the prediction steps for the different methods. The used parameters are: [G-VARMA \eqref{eq:joint_causal_model} : $P = 1$, $Q = 1$, $\sigma_{\text{s}} = 0.5$ \elvin{There should be another parameter here, right?}], [GP-VAR: $P = 1$, $L_p = L = 4$, $\sigma_{\text{s}} = 0.5$], [ARMA: $P = 1$, $Q = 0$], [RGP-VAR \cite{mei2017signal}: $P = 2$], [LMS on Graphs  \cite{di2016adaptive}: B.width $= 16$, $\mu_{\text{LMS}} = 1.4$], [RLS on Graphs \cite{di2017adaptive}: B.width $=16$, $\beta_{\text{RLS}} = 0.05$].}
%\label{fig.epid_pred_pow}
%\end{figure}

%Additionally, we make also the following remarks. First, the prediction rNMSE is slightly higher in this data set w.r.t. the previous two cases. We attribute this performance degradation to the ``abrupt" signal transition in the patient recovery instances (i.e., every $12$ days). Secondly, here we observe that the G-VARMA models has coefficients also in the MA part, while in the previous two examples it reduced to a G-VAR model. This behavior is transcendent from the used amount of in-sample and training data. In fact, even for the other two data sets we have achieved full G-VARMA models with a different percentage of training samples. Finally, we consistently observed that the chosen models are characterized by a bounded memory in time. That is, only few past realizations are useful for the prediction task. Contrarily, the proposed GP-VAR model shows that there is a larger graph influence in the prediction model. Indeed, information from nodes up to four hops away is exploited in Fig.~\ref{fig.epid_pred_pow} and also in Fig.~\ref{fig.mol_pred_pow}.

%\begin{figure}[t]
%\centering
%\includegraphics[width=\columnwidth,trim={.4cm 0 .7cm .35cm},clip]{figures/e_Epid_predVal13.pdf}
%\caption{Evolution of the infection portion and the G-VARMA one and three steps ahead predictions on all the graph.}
%\label{fig.epid_true_sig}
%\end{figure}
%
%To conclude, Fig.~\ref{fig.epid_true_sig} shows the evolution of the infected state on all the graph and the respective G-VARMA predictions. Generally, we observe that the proposed model follows relatively well the (I) state evolution with a prediction error of $3\%$ in the one-step-ahead and $6\%$ in the three steps ahead predictions.
%
%\vskip 1mm
%\noindent\textbf{In-sample data effect.}


==> journal revised/section_prelim.tex <==
%!TEX root = main.tex

This section starts with the fundamentals of graph and time-vertex signal processing. Then, it proceeds with the two-dimensional time-vertex ARMA models and the definition of joint stationarity that will be used in the rest of the paper.

%---------------------------------------------------------------------------------------------------
%---------------------------------------------------------------------------------------------------
\subsection{Graph Signal Processing}
\label{subsec_gsp}

Consider a weighted undirected graph $\Gr = (\Vx,\Ed,\W_\Gr)$, where $\Vx$ is the set of $N$ nodes (vertices), $\Ed$ is the edge set, and $\W_\Gr$ is the weighted adjacency matrix with $[\W_\Gr]_{ij} = [\W_\Gr]_{ji} > 0$ if $(i,j) \in \Ed$ and zero otherwise. A graph signal is a mapping from the vertex set to the set of complex numbers, \ie x $: \Vx \to \mathbb{C}$. For convenience we represent a graph signal by the vector $\x = [x_1,\ldots , x_N]^{\transp}$, where $x_i$ is the value related to node $i$. The graph Fourier transform (GFT) of $\x$ is
%
\begin{equation}
\label{eq.gft}
\GFT{\x} = \U_\Gr^\herm\x,
\end{equation}
where $\U_\Gr$ is the unitary eigenvector matrix of the discrete Laplacian matrix $\L_\Gr = \text{diag}(\W_\Gr\mathbf{1}_N) - \W_\Gr = \U_\Gr\LAM_\Gr\U_\Gr^\herm$. The diagonal matrix $\LAM_\Gr$ contains the eigenvalues on its main diagonal, often referred to as the graph frequencies \cite{Shuman2013}. The GFT allows filtering on graphs in the graph frequency domain. The filtered version $\y$ of $\x$ with the graph filter $h(\L_\Gr) \in \mathbb{R}^{N\times N}$ corresponds to an element-wise multiplication in the spectral domain, \ie
%
%
\begin{equation}
    \y = h(\L_\Gr)  \x \triangleq \U_\Gr h(\LAM_\Gr) \U_\Gr^\herm \, \x, 
\end{equation}
%
with matrix $h(\L_\Gr)$ obtained by applying the scalar function $h: [0, \lambda_{\textit{max}}] \rightarrow \Rbb$ on the eigenvalues of $\L_\Gr$. Here, $h(\LAM_\Gr)$ is diagonal and is referred to as the graph filter frequency response. See \cite{taubin2000geometric,Shuman2013,sandryhaila2013discrete} for more details on GSP and \cite{shuman2011chebyshev,Shi2015, segarra2017optimal,isufi2017autoregressive} for graph filters.

%---------------------------------------------------------------------------------------------------
%---------------------------------------------------------------------------------------------------
\subsection{Time-Vertex Signal Processing}
\label{subsec_gtsp}

For a time-varying graph signal $\x_t$, let $\X_{1:T} = [\x_1, \x_2, \ldots, \x_T] \in \mathbb{R}^{N \times T}$ be the $N \times T$ matrix that collects $T$ successive realizations. Let also $\x_{1:T} = \text{vec}(\X_{1:T})$ denote the vectorized form of $\X_{1:T}$. From \cite{grassi2017time}, the joint (time-vertex) Fourier transform (JFT) of $\X_{1:T}$ is
%
%
\begin{align}
\label{eq.jft_def}
    \JFT{\X_{1:T}} = \U_\Gr^{\herm} \X_{1:T} {\U}_{\mathcal{T}}^*,
\end{align}
%
where, once again $\U_\Gr$ is the graph Laplacian eigenvector matrix, \rev{while ${\U}_{\mathcal{T}}^* \in \mathbb{C}^{T\times T}$ is the complex conjugate} of the discrete Fourier transform (DFT) matrix. $\U_{\mathcal{T}}$ can also be interpreted as the unitary eigenvector matrix of the circulant time-shift operator $\L_{\mathcal{T}} = \U_{\mathcal{T}} \, \LAM_{\mathcal{T}} \, \U_{\mathcal{T}}^\herm$\rev{
%
\begin{equation}
[\LAM_{\mathcal{T}}]_{tt} = e^{-\j \omega_t}, \quad \text{and}\quad \omega_t = \frac{2\pi (t-1)}{T}
\end{equation}
%
for $\j = \sqrt{-1}$ and $t = 1, \ldots, T$}. In a vectorized form, \eqref{eq.jft_def} becomes $\JFT{\x_{1:T}} = \U_{\mathcal{J}}^\herm\x$, with $\U_{\mathcal{J}} = \U_{\mathcal{T}}\otimes\U_\Gr$ being a unitary matrix.

Similar to the GFT, the JFT allows a \emph{joint} time-vertex filtering of $\x_{1:T}$ in the joint time-vertex frequency domain. The latter is given by the eigendecomposition of the extended Laplacian operator $\L_{\mathcal{J}} = \I_N \otimes \L_\Gr + \L_{\mathcal{T}}\otimes \I_N$ \cite{grassi2017time}. The joint filtered version $\y_{1:T}$ of $\x_{1:T}$ with a joint filter $h(\L_{\mathcal{J}})$ corresponds again to an element-wise multiplication, but now in the joint frequency representation, i.e.,
%
%
\begin{equation}  \label{eq:def_joint_filtering}
    \y_{1:T} = h(\L_{\mathcal{J}}) \x_{1:T} \triangleq \U_{\mathcal{J}} \, h(\LAM_\Gr, \LAM_{\mathcal{T}} ) \, \U_{\mathcal{J}}^\herm \x_{1:T}. %vec(\UG \left(h(\bLambda_G,\bOmega)\circ(\UG^* \X \bar{\U}_T)\right)\UT^\transpose)
\end{equation} 
%
{Here, $h(\LAM_\Gr,\LAM_{\mathcal{T}})$ is an $NT\times NT$ diagonal matrix called the joint time-vertex frequency response with $k$th diagonal element $[h(\LAM_\Gr,\LAM_{\mathcal{T}})]_{kk} = h(\lambda_n,e^{\j\omega_t})$ and $k = N(t-1)+n$ for $n = 1, \ldots, N$ and $t = 1, \ldots, T$.} By means of inverse vectorization, we write $\Y_{1:T} = \textnormal{vec}^{-1}(\y_{1:T})$ and the $t$th column of $\Y_{1:T}$, $\y_t$, is the filtered signal at time $t$. %Refer to \cite{grassi2017time} for further detail.

\vspace{2mm}\noindent\textbf{Time-vertex ARMA filters.} An efficient way to (distributively) implement \eqref{eq:def_joint_filtering} is by extending the two-dimensional ARMA filters \cite{Isufi2016separable} to the more general form
%
\begin{equation}
\label{eq.2dARMA}
\y_t + \sum_{p = 1}^P\sum_{l = 0}^{L_p}\psi_{l,p}\L_\Gr^l\y_{t-p}= \sum_{q = 0}^Q\sum_{k=0}^{K_q}\varphi_{k,q}\L_\Gr^k\x_{t-q},
\end{equation}
where $P, L_p, Q, K_q$ are positive scalars and $\psi_{l,p}, \varphi_{k,q}$ denote complex coefficients. In computing the filter output $\y_t$, recursion \eqref{eq.2dARMA} considers a linear combination of the current and past graph signal realizations $\{\x_{t}, \ldots, \x_{t-Q}\}$ and of the previous outputs $\{\y_{t-1}, \ldots, \y_{t-P}\}$. This temporal shifting of the filter input-output provides a filtering in the temporal domain. The graph filtering is provided by shifting each temporal realization $\x_{t-\tau}$ ($\y_{t-\tau}$) in the graph dimension using powers of $\L_\Gr$.

To see more formally the two-dimensional filtering effect of \eqref{eq.2dARMA}, we first apply the DFT and then the GFT on both sides of \eqref{eq.2dARMA} to obtain the per time-vertex frequency relation
%
\begin{align}
\label{eq.2dARMA_freq}
\left(\!\!1 \!+\!\! \sum_{p = 1}^P\sum_{l = 0}^{L_p}\psi_{l,p}\lambda_n^le^{-\j \omega_t p}\right)\hat{y}_{n}(e^{\j\omega_t}) &= \notag \\
&\hspace{-25mm}\sum_{q = 0}^Q\sum_{k=0}^{K_q}\varphi_{k,q}\lambda_n^le^{-\j \omega_t q}\hat{x}_{n}(e^{\j\omega_t}),
\end{align}
where $\hat{y}_{n}(e^{\j\omega_t})$ ($\hat{x}_{n}(e^{\j\omega_t})$) is the $n$th entry of $\GFT{\DFT{\y_t}}$ ($\GFT{\DFT{\x_t}}$). Then, for stable filter coefficients $\psi_{l,p}$, \ie coefficients that abide to 
%
%which for stable filter coefficients $\psi_{l,p}$, \ie coefficients that abide to 
%
\begin{equation}
\label{eq.2dARMA_stable}
1 + \sum_{p = 1}^P\sum_{l = 0}^{L_p}\psi_{l,p}\lambda_n^le^{-\jmath \omega_t p} \neq 0, \quad \forall~ n = 1, \ldots, N,
\end{equation}
\eqref{eq.2dARMA} implements the two-dimensional time-vertex frequency response
%
\begin{equation}
\label{eq.2dARMA_fresp}
h(\lambda_n,e^{\j \omega_t}) = \frac{\sum_{q = 0}^Q\sum_{k=0}^{K_q}\varphi_{k,q}\lambda_n^ke^{-\j \omega_t q}}{1 + \sum_{p = 1}^P\sum_{l = 0}^{L_p}\psi_{l,p}\lambda_n^le^{-\j \omega_t p}}.
\end{equation}
It is easy to see that the above frequency response is a joint time-vertex filter. 
%
Similarly to its separable counterpart \cite{Isufi2016separable}, recursion \eqref{eq.2dARMA} considers polynomial shifting in the graph dimension. Thus, from the locality of $\L_\Gr$ \cite{Shuman2013}, and since $\L_\Gr^k\x_{t-q} = \L_\Gr(\L_\Gr^{k-1}\x_{t-q})$ \cite{shuman2011chebyshev,segarra2017optimal}, recursion \eqref{eq.2dARMA} enjoys the same distributed implementation as \cite{Isufi2016separable}.

We conclude this section with the following observation.

\begin{remark}[Model generality] Recursion \eqref{eq.2dARMA} encompasses some of the state-of-the-art two-dimensional time-vertex models. Specifically:
%
\begin{itemize}
\item for $\psi_{l,p} = \psi_la_p$ and $\varphi_{p,q} = \varphi_pb_q$ it specializes to the separable case~\cite{Isufi2016separable};
\item for $\psi_{l,p} = 0$ $\forall l, p$, it boils down to the two-dimensional finite impulse response time-vertex filter~\cite{Isufi2016Dim2};
\item for $L_p = p$, $\sum_{k=0}^{K_0}\varphi_{k,0}\L_\Gr^k = \I_N$ and $\varphi_{k,q} = 0$ otherwise, it reduces to the model of \cite{mei2017signal}.
\end{itemize}
\end{remark}

In Section~\ref{subsec_jcmg} we exploit recursion \eqref{eq.2dARMA} to model network processes for the task of prediction. This will allow us to exploit its polynomial implementation, and thus provide a distributed predictor.

%---------------------------------------------------------------------------------------------------
%---------------------------------------------------------------------------------------------------
\subsection{Stationarity on Networks}
\label{subsec_stat}

Stationarity is another useful property that extends to graph signals \cite{Girault2015,Perraudin2016,Marques2016} and allows performing graph Wiener filtering/interpolation and spectral estimation. \rev{From the analogies with the concept of stationarity in time signals, graph stationarity requires that the signal first and second order moments are preserved along the graph dimension.} Limiting ourselves to zero-mean processes, one way to define graph wide-sense stationarity (GWSS) is:

\begin{definition}[GWSS]\label{def.gwss} A random graph process $\x$ is wide-sense stationary, if and only if its covariance matrix $\bSigma_x = \Exp[\x\x^\herm]$ is diagonalizable by the GFT basis $\U_\Gr$, \ie $\bSigma_x = \U_\Gr\textnormal{diag}(\p_x)\U_\Gr^{\herm}$. The $N \times 1$ vector $\p_x$ is the GFT of the autocorrelation function of $\x$ and is referred to as the graph power spectral density.% (GPSD).
\end{definition}

This condition imposes the invariance of the second order statistics w.r.t. a translation using the shift operator $\L_\Gr$. \rev{That is, as for time signals the second order moment is invariant to temporal translations, here, the invariance of the graph signal statistics should also account for the underlying structure. Moreover, similar to classical temporal stationarity, a useful property of GWSS signals is that $\x$ can be driven by a graph filter applied to a zero-mean white noise.} The graph filter $h(\LAM_\Gr)$ should then satisfy $|h(\LAM_\Gr)|^2 = \text{diag}(\p_x)$.

In analogy with the definition of the JFT, stationarity can be extended to time-varying graph processes \cite{loukas2016stationary}. \rev{This new concept of stationarity requires now that the first and second order moments are jointly  preserved along the graph and temporal dimension.} Limiting ourselves again to zero-mean processes, joint wide-sense stationarity (JWSS) can be defined as follows:

%
\begin{definition}[JWSS]\label{def.jwss}
A random time-vertex process $\x_{1:T} = \textnormal{vec}(\X_{1:T})$ is called jointly (or time-vertex) wide-sense stationary, if and only if its covariance matrix $\bSigma_{x_{1:T}} = \Exp[\x_{1:T}\x_{1:T}^\herm]$ is diagonalizable by the JFT basis $\U_{\mathcal{J}}$, \ie $\bSigma_{{1:T}} =  \U_{\mathcal{J}}\textnormal{diag}(\p_{{1:T}})\U_{\mathcal{J}}^{\herm}$. The $NT\times 1$ vector $\p_{{1:T}}$ is the JFT of the autocorrelation function of the process $\x_{1:T}$ and is referred to as joint power spectral density (JPSD). 
\end{definition}
%
%\andreas{We could rename $\bSigma_{x_{1:T}}$ to $\bSigma_{1:T}$ and same for $\p$}

With this definition, one now assumes simultaneously wide-sense stationarity w.r.t. both the \emph{time} and \emph{vertex} domains. This condition requires now invariance w.r.t. translation using the joint time-vertex shift operator. Further, for a JWSS time-vertex process the covariance is now related to a joint filter $h(\LAM_\Gr,\LAM_{\mathcal{T}})$. Specifically, $\x_{{1:T}}$ can be driven by time-vertex filtering zero-mean white noise, where $h(\LAM_\Gr,\LAM_{\mathcal{T}})$ must now satisfy $|h(\LAM_\Gr,\LAM_{\mathcal{T}})|^2 = \text{diag}(\p_{{1:T}})$.

%In the sequel, we will make use of the JWSS present in real data---{not often observed as in time but good enough for prediction}--- to answer the question: ``\textit{How to construct models that concisely capture the characteristics of a jointly stationary process, in order to facilitate short-term prediction?}''.





==> journal revised/section_subset.tex <==
% !TEX root = main.tex
\begin{figure}
\centering
\includegraphics[width=0.8\columnwidth]{figures/graph_observed.png}
\caption{Illustration of the sampling set and its complementary set. The black nodes are observed at time $t$, while the white nodes are not accessed. At previous time instants, all nodes are observed.}
\label{fig.ill_graph}
\end{figure}

This section looks at estimating $\x_t$ by using both the historical data and measurements at time $t$ collected on a subset $\Scal_t \subseteq \Vx$ of nodes. In what follows, we consider the G-VARMA model to address this task. At the end of this section, we remark how the tracking can be addressed by other models.

A possible application involving this scenario comprises a survey outcome in a social network. Here, it is likely that a (possibly significant) number of users do not take part in the survey after a certain time instant.
%
%We identify two possible applications involving this scenario. The first is a survey outcome in a social network where a (possibly significant) number of users do not take part in the survey after a certain time instant. 
By using the developed predictors and the observations on $\Scal_t$, we are interested to estimate the survey outcome at time $t$ on another set $\bar{\Scal}_t$. %The second application consists of tracking the signal evolution on a sensor network. Due to energy constraints, some sensors are set in standby. We then aim estimating $\x_t$ on all (or part of) the nodes from both the historical data and the measurements in $\Scal_t$. 
The set $\bar{\Scal}_t$ might then be: $(i)$ $\bar{\Scal}_t = \Vx$, i.e., improve the estimation on all nodes; $(ii)$ $\bar{\Scal}_t = \Vx\backslash\Scal_t$, i.e., the complementary set of $\Scal_t$; or $(iii)$ a combination on the two. Fig.~\ref{fig.ill_graph} illustrates one such example.

Let $\D_t \in \{0,1\}^{|\Scal_t|\times N}$ be a binary matrix containing the non-zero rows of $\D_{\Scal_t} = \text{diag}(\mathbf{1}_{\Scal_t})$. Note that by construction $\D_t\D_t^\transp = \I_{|\Scal_t|}$ and $\D_t^\transp\D_t = \D_{\Scal_t}$. Similarly, let $\bar{\D}_t$ be the $|\bar{\Scal}_t| \times N$ binary matrix relative to the set $\bar{\Scal}_t$.
%
%
%Let us denote $\D_\Scal = \text{diag}(\mathbf{1}_\Scal)$ as the diagonal matrix that projects onto the observed set $\Scal$, and $\D_{\Scal_c} = \I_N - \D_\Scal$ as the diagonal matrix that projects onto the complementary set $\Scal_c$. Observe that by construction both $\I_\Scal$ and $\I_{\Scal_c}$ are idempotent matrices. 
%To better enhance the benefits of this analysis we rely on the following assumption:
%
%\begin{assumption}\label{ass_blim}
%The G-VARMA kernel matrices $a_p(\L_\Gr)$ and $b_q(\L_\Gr)$ are estimated from a $K$-rank model as described in Theorem~\ref{theo.low_rank}.
%\end{assumption}
%\noindent This assumes the parameters to be estimated only on a subset of the graph frequencies, and thus the causal model is (approximately) graph-bandlimited. Besides easing the estimation costs, Assumption~\ref{ass_blim} is often met in practice, see for instance \cite{di2017adaptive,isufi2017observing}.
%
%In the sequel, we use the G-VARMA model and Assumption~\ref{ass_blim} to address the task of tracking on a subset of nodes.
Let also $\z_t = \D_t(\x_t + \w_t)$ be the $|\Scal_t| \times 1$ vector of measurements at time $t$ with $\w_t$ the zero-mean measurement noise with covariance matrix $\bSigma_w$ independent from $\boldsymbol{\varepsilon}_t$. Then, for $\x_t$ following the G-VARMA model \eqref{eq:joint_causal_model}, we have
%
\begin{equation}
\z_t = \D_t \eps_t + \D_t\tilde{\x}_{t} + \D_t\w_t,
\end{equation}
%
with $\tilde{\x}_{t}$ from \eqref{eq:predictor1}. The linear minimum mean square estimate (LMMSE) for $\eps_t$ is
%
\begin{align}\label{eq.lmmse1}
\tilde{\eps}_t &=  \bSigma_{\varepsilon}\D_t^\transp \H_t^{-1}(\z_t - \D_t\tilde{\x}_{t}),
\end{align}
%
where $\H_t = \D_t\left(\bSigma_{\varepsilon} + \bSigma_w\right)\D_t^\transp$ \cite{kay1993fundamentals}. Substituting $\tilde{\eps}_t$ into the signal evolution over the set $\bar{\Scal}_t$, we get
%
\begin{align}\label{eq.lmmse_fin}
	\tilde{\x}_{\bar{\Scal},t} = \bar{\D}_t \bigg(\tilde{\x}_{t} + \bSigma_{\varepsilon}\D_t^\transp \H_t^{-1}(\z_t - \D_t\tilde{\x}_{t}) \bigg). 
\end{align}
%
This is the estimate of $\x_t$ on $\bar{\Scal}_t$ which considers the G-VARMA prediction $\tilde{\x}_t$ and the measurements collected over $\Scal_t$. Estimator \eqref{eq.lmmse_fin} considers, in addition to its past realizations, i.e., $ \bar{\D}_t\tilde{\x}_{t}$, an inverse filtering on the observed vertices and then a spreading onto the set $\bar{\Scal}_t$.

Following the KF convention \cite{simon2006optimal}, $\tilde{\x}_{\bar{\Scal},t}$ in \eqref{eq.lmmse_fin} is the \emph{a posteriori} estimate of $\x_t$ on the set of interest $\bar{\Scal}_t$ and $\tilde{\x}_{t}$ is the \emph{a priori} estimate of $\x_t$. The latter allows then to easily quantify in closed form the MSE of estimator \eqref{eq.lmmse_fin}. In fact, given the \emph{a priori} error covariance matrix over $\mathcal{V}$, $\P_t^- = \bSigma_\varepsilon$, and the \emph{a posteriori} error covariance matrix over ${\bar{\Scal}_t}$
%
\begin{equation}
\label{eq.pos_cov_mat}
\P_{\bar{\Scal},t}^+ = \bar{\D}_t(\I_N - \K_t\D_t)\P_t^-\bar{\D}_t^\transp,
\end{equation}
%
with Kalman gain matrix
%
\begin{equation}\label{eq.KalGain}
\K_t = \P_t^-\D_t^\transp\H_t^{-1},
\end{equation}
%
the MSE of \eqref{eq.lmmse_fin} is
%
\begin{align}\label{eq.MSE_subset}
\begin{split}
\textit{MSE} &= \Exp\bigg[\|\x_{\bar{\Scal},t} - \bar{\D}_t\x_t	\|_2^2	\bigg]\\
&=\trace\bigg(\bar{\D}_t(\I_N - \bSigma_\varepsilon\D_t^\transp\H_t^{-1}\D_t) \bSigma_\varepsilon\bar{\D}_t^\transp	\bigg),
\end{split}
\end{align}
%
with $\H_t$ defined in \eqref{eq.lmmse1}.

The MSE \eqref{eq.MSE_subset} shows the dependence of the reconstruction performance on the sampling set (through $\D_t$) and the G-VARMA model (through the residual error $\bSigma_\varepsilon$). To select the sampling set $\Scal_t$, we can exploit the above KF reformulation of \eqref{eq.lmmse_fin} and use the sparse-sensing sampling strategies \cite{chepuri2016sparse} adopted in \cite{isufi2017observing} for tracking diffusion processes on graphs. However, as found in the latter work, the MSE would improve by $1$dB-$2$dB w.r.t. a random uniform sampling. While the latter can be used (at the expense of a higher complexity), in this work we show the potential of the proposed tracker by building $\Scal_t$ uniformly at random.

%%---------------------------------------------------------------------------------------------------
%%---------------------------------------------------------------------------------------------------
%\subsection{Tracker}
%\label{subsec_pred}
%Let $\z_t = \D_t(\x_t + \w_t)$ be the $|\Scal_t| \times 1$ vector of measurements at time $t$ with $\w_t$ a zero-mean noise with covariance matrix $\bSigma_w$. Then, for $\x_t$ following the G-VARMA model \eqref{eq:joint_causal_model}, we have
%\begin{equation}
%\z_t = \D_t b_0(\L_\Gr)\eps_t + \D_t\tilde{\x}_{t} + \D_t\w_t,
%\end{equation}
%with $\tilde{\x}_{t}$ from \eqref{eq.one_stepPred}. The linear minimum mean square estimate (LMMSE) for $\eps_t$ is given by \cite{kay1993fundamentals}:
%\begin{align}\label{eq.lmmse1}
%\tilde{\eps}_t &=  b_0^\herm(\L_\Gr)\D_t^\herm \H_t^{-1}(\z_t - \D_t\tilde{\x}_{t}),
%\end{align}
%where $\H_t = \big(\D_t b_0(\L_\Gr)b_0^\herm(\L_\Gr)\D_t^\herm + \D_t\bSigma_w\D_t^\herm\big)$. Substituting $\tilde{\eps}_t$ into the signal evolution over the set $\bar{\Scal}_t$, we get
%%
%\begin{align}\label{eq.lmmse_fin}
%	\tilde{\x}_{\bar{\Scal},t} = \bar{\D}_t \left(\tilde{\x}_{t} +  b_0(\L_\Gr)b_0^\herm(\L_\Gr)\D_t^\herm \H_t^{-1}(\y_t - \D_t\tilde{\x}_{t}) \right).
%\end{align}
%%
%This is the estimate of $\x_t$ on $\bar{\Scal}_t$ which considers the G-VARMA prediction $\tilde{\x}_t$ and the measurements collected over $\Scal_t$. 
%
%Estimator \eqref{eq.lmmse_fin} considers, in addition to its past realizations, i.e., $ \bar{\D}_t\tilde{\x}_{t}$, an inverse filtering on the observed vertices and then a spreading onto the set $\bar{\Scal}_t$.
%
%{From \eqref{eq.lmmse_fin}, note that the measurement set $\Scal_t$ plays an important role in the attained LMMSE as it affects the rank of $\H_t$. Let us momentarily consider the noiseless case, where $\w_t = \mathbf{0}_N$. Then, $\H_t$ is of full rank $K$ only if rank$(\D_t) = K$ (recall rank$(b_0(\L_\Gr)) = K$ under Assumption~\ref{ass_blim}).
%%
%Therefore, a necessary condition guaranteeing the full rank of $\H_t$ is: %for estimating $\x_{\bar{\Scal},t}$ from the measurements taken on $\Scal_t$ is:
%%
%\begin{equation}
%\label{eq.prop_sub_pred}
%|\Scal_t| \ge K.
%\end{equation}
%%
%That is, the cardinality of the sampling set must be greater than or equal to the dimension of the process low-rank representation. However, \eqref{eq.prop_sub_pred} is not sufficient since $\H_t$ may be rank deficient depending on the sampled nodes leading often to large reconstruction MSE.}

%In the sequel, we provide a Kalman filtering (KF) on graph interpretation for the above derivations which allows us to leverage well-established results for its MSE analysis.
%
%%---------------------------------------------------------------------------------------------------
%%---------------------------------------------------------------------------------------------------
%\subsection{Interpretation as Kalman Filtering on Graphs}
%\label{subsec_subMSE}
%
%The predictor in Section~\ref{sec.mod} was $$\tilde{\x}_t = \Exp\bigg[\x_t \bigg| \{\x_1, \ldots, \x_{t-1}\}\bigg],$$ for a set of training data $\{\x_1, \ldots, \x_{t-1}\}$. %where $\z_\tau$ stems for the training data. 
%%
%Following the KF notation \cite{simon2006optimal}, $\tilde{\x}_t$ is the \emph{a priori} estimate of $\x_t$ (i.e., before we process the measurement at time $t$) denoted as $\tilde{\x}_t^- = \tilde{\x}_t$. Proposition~\ref{prop:mse_1step} characterized the \emph{a priori} error covariance matrix $\P_t^- = b_0(\L_\Gr)b_0(\L_\Gr)^\herm$ for $\tilde{\x}_t^-$.
%
%With this in place, the Kalman gain matrix due to $\z_t$ is
%%
%\begin{equation}\label{eq.KalGain}
%\K_t = \P_t^-\D_t^\herm(\D_t\P_t^-\D_t^\herm + \D_t\bSigma_w\D_t^\herm)^{-1},
%\end{equation}
%leading to the all-node \emph{a posteriori} estimate:
%%
%\begin{align}
%\label{eq.post_KF}
%\begin{split}
%\tilde{\x}_t^+ = \tilde{\x}_t^- + \K_t (\y_t - \D_t\tilde{\x}_t^-).
%\end{split}
%\end{align}
%%
%The \emph{a posteriori} estimate on the set of interest $\bar{\Scal}_t$ is $\tilde{\x}_{\bar{\Scal},t}^+ = \bar{\D_t}\tilde{\x}_t^+$, which after substituting $\tilde{\x}_t^-$, $\K_t$ and $\P_t^-$ becomes identical to \eqref{eq.lmmse_fin}.
%
%The above KF reformulation of \eqref{eq.lmmse_fin} leads to several insights about the introduced tracking scheme. It shows the optimality of \eqref{eq.lmmse_fin} in incorporating the measurements at time $t$ into the estimation of $\x_{\bar{\Scal},t}$. Further, it highlights the versatility of the proposed formulation on time-varying network processes. In fact, no assumption on the particular process evolution of $\x_t$ is made (that is, apart from the process being low-rank and stationary), which is not common ground for signal tracking through Kalman filters. Finally, it allows us to quantify the MSE of \eqref{eq.lmmse_fin} from the well-established KF theory.
%%
%
%The MSE of $\x_{\bar{\Scal},t}$ is
%%
%\begin{align}\label{eq.MSE_subset}
%\begin{split}
%\textit{MSE} &= \Exp\bigg[\|\x_{\bar{\Scal},t} - \bar{\D}_t\x_t	\|_2^2	\bigg] = \Exp\bigg[\|\bar{\D_t}\tilde{\x}_t^+ - \bar{\D}_t\x_t\|_2^2	\bigg]\\
%&=\trace\bigg(\bar{\D}_t\Exp\bigg[\big(\tilde{\x}_t^+ - \x_t	\big)\big(\tilde{\x}_t^+ - \x_t	\big)^\herm\bigg]\bar{\D}_t^\herm\bigg).
%\end{split}
%\end{align}
%In \eqref{eq.MSE_subset}, note that $\Exp\bigg[\big(\tilde{\x}_t^+ - \x_t	\bigg)\big(\tilde{\x}_t^+ - \x_t	\bigg)^\herm\bigg]$ is the \emph{a posteriori} error covariance matrix $\P_t^+$ which has the closed form expression
%
%\begin{equation}
%\label{eq.pos_cov_mat}
%\P_t^+ = (\I_N - \K_t\D_t)\P_t^-.
%\end{equation}
%Then, by plugging \eqref{eq.pos_cov_mat} back into \eqref{eq.MSE_subset} and substituting $\K_t$ and $\P_t^-$ we get
%
%\begin{align}\label{eq.MSE_subset1}
%\begin{split}
%\textit{MSE} &= \trace\bigg(\bar{\D}_t(\I_N - b_0(\L_\Gr)b_0(\L_\Gr)^\herm\D_t^\herm\H_t^{-1}\D_t)\\
%&\qquad\qquad \times b_0(\L_\Gr)b_0(\L_\Gr)^\herm\bar{\D}_t^\herm	\bigg),
%\end{split}
%\end{align}
%with $\H_t$ defined in \eqref{eq.lmmse1}.
%
%The MSE \eqref{eq.MSE_subset} shows the dependence of the reconstruction performance on the sampling set (through $\D_t$) and the G-VARMA model (through $b_0(\L_\Gr)$). To select the sampling set $\Scal_t$, we can exploit the above KF reformulation of \eqref{eq.lmmse_fin} and use the sparse-sensing sampling strategies \cite{chepuri2016sparse} adopted in \cite{isufi2017observing} for tracking diffusion processes on graphs. However, as found in the latter work, the MSE would improve by $1$dB-$2$dB w.r.t. a random uniform sampling. While the latter can be used (at the expense of a higher complexity), in this work we show the potential of the proposed tracker by building $\Scal_t$ uniformly at random.





%%---------------------------------------------------------------------------------------------------
%%---------------------------------------------------------------------------------------------------
%\subsection{Mean Square Error Analysis}
%\label{subsec_subMSE}
%To compute the MSE for \eqref{eq.gc_varma_subgr4} we first note that for $\eps_t$ belonging to some distribution $\mathcal{P}(\mathbf{0}, \I_N)$, it implies $\x_t\sim\mathcal{P}(\c_{t-1}, \bSigma_{x,t}=b_0(\L_\Gr)b_0(\L_\Gr)^\herm)$. Further, from \eqref{eq.gc_varma_subgr4} $\Exp(\D_{\Scal_c}\x_t) =  \D_{\Scal_c}\c_{t-1}$. Then, the following proposition quantifies the MSE of the subgraph predictor \eqref{eq.gc_varma_subgr4}.
%
%\begin{proposition}\label{prop.mse_subgr}
%The MSE of the predicted value on the set $\Scal_c$ with the subgraph predictor \eqref{eq.gc_varma_subgr4} is
%
%\begin{align}\label{eq:MSE_subgr}
%\begin{split}
%MSE &= \trace\Bigg(\bSigma_{x,t} + \c_{t-1}\c_{t-1}^\herm		\Bigg) - \trace\Bigg(\D_{\Scal}\Big(\bSigma_{x,t}+ \c_{t-1}\c_{t-1}^\herm	\Big)\Bigg)\\
%& + \trace\left(b_0(\L_\Gr)^\herm b_0(\L_\Gr)\left(b_0(\L_\Gr)^\herm\D_{\Scal}b_0(\L_\Gr)	\right)^{-1}	\right) - N.
%%
%%
%%\trace\left(b_0(\L_\Gr)^\herm b_0(\L_\Gr)\left(b_0(\L_\Gr)^\herm\I_{\Scal}b_0(\L_\Gr)	\right)^{-1}	\right) - N + \trace\Bigg(\bSigma_{x,t} -  \I_{\Scal}\bSigma_{x,t}	\Bigg)\\
%%&\qquad + \trace\left(\c_{t-1}\c_{t-1}^\herm	-\I_{\Scal}\c_{t-1}\c_{t-1}^\herm\right),
%\end{split}
%\end{align}
%\end{proposition}
%\andreas{There is some error here: what you have in the parenthesis in not invertible (since $\D_\Scal$ is not full rank). Otherwise, we would have $\trace( b_0(\L_\Gr)^\herm b_0(\L_\Gr)\left(b_0(\L_\Gr)^\herm\D_{\Scal}b_0(\L_\Gr)	\right)^{-1}) = \trace(\D_{\Scal}^{-1})$ Maybe use pseudo-inverse?}.
%
%The latter result yields two meaningful insights. First, through $\D_\Scal$ we observe the impact of the sampling set on the subgraph predictor MSE. Secondly, the graph topology embedded in $b_0(\L_\Gr)$ plays a role in the MSE performance as well. Thus, we may conclude that not only the number of sampled nodes plays a role, but also their position w.r.t. the underlying graph.
%
%In the next section, we propose a node sampling strategy (if the problem allows that) to carefully reconstruct the set $\Scal$ by guaranteeing a target MSE performance.
%
%%---------------------------------------------------------------------------------------------------
%%---------------------------------------------------------------------------------------------------
%\subsection{Sampling Strategy}
%\label{subsec_sampl}
%
%Here, we introduce an optimal node sampling strategy to construct the set $\Scal$ that contains the minimal number of vertices, such that a target MSE prediction performance on $\Scal_c$ is guaranteed. Following a sparse sensing approach \cite{joshi2009sensor,chepuri2015sparsity}, we denote as $\w = [w_1, \ldots, w_N]^\transp$ the node selection vector with $w_i = 1$ if $v_i \in \Scal$ and $w_i = 0$, otherwise. With this in place, the MSE \eqref{eq:MSE_subgr} can be written as
%
%\begin{align}\label{eq.mse_subgr_w}
%\begin{split}
%MSE(\w) &= \trace\left(b_0(\L_\Gr)^\herm b_0(\L_\Gr)\left(b_0(\L_\Gr)^\herm\text{diag}(\w)b_0(\L_\Gr)	\right)^{-1}	\right)\\
%&\quad+\trace\Bigg(\bSigma_{x,t} + \c_{t-1}\c_{t-1}^\herm		\Bigg) -N\\
%& \quad- \trace\Bigg(\text{diag}(\w)\Big(\bSigma_{x,t}+ \c_{t-1}\c_{t-1}^\herm	\Big)\Bigg),
%\end{split}
%\end{align}
%which then allows us to rephrase the selection problem as
%
%\begin{align}
%\begin{split}
%&\underset{\w}{\text{minimize}}~~\mathbf{1}^\transp\w\\
%&\text{subject to}~~  MSE(\w) \le \gamma\\
%&\hskip19mm w_n \in [0,1],~\forall~n=1, \ldots, N.
%\end{split}
%\label{eq.node_selection}
%\end{align}
%%
%\andreas{This is not necessarily optimal.. (in compressive sensing one needs a specific number of measurements that depends on the sparsity).}
%Problem~\eqref{eq.node_selection} is already the relaxed version of the NP-hard sensor selection counterpart and can be efficiently solved via numerical tools such as CVX \cite{grant2008cvx}. Specifically, the objective function is the surrogate of the $l_0$-norm and imposes sparsity in the set $\Scal$. The first constraint imposes a target MSE prediction performance $\gamma$ on the complementary set $\Scal$, while the second constraint is a relaxation of the Boolean set (i.e., $w_i \in \{0,1\},~i = 1, \ldots, N$)  to the box one \cite{joshi2009sensor}.
%
%Conversely, one can also consider the opposite problem, i.e., minimizing the MSE such that a fixed number of nodes $|\Scal| = K$ is selected. The latter can also be relaxed in a convex problem as well. Finally, once the optimal solution $\w^*$ of \eqref{eq.node_selection} is obtained, thresholding, or randomized rounding can be performed to project $\w^*$ to the Boolean set $\{0,1\}^N$ and construct $\Scal$.

%Before proceeding with the numerical results, we make the following observation.

%We conclude the our theoretical analysis with the following observation.

\begin{remark}[Other models] As the KF interpretation highlighted, estimator \eqref{eq.lmmse_fin} uses $\P_t^- = \bSigma_\varepsilon$ of G-VARMA to connect the prediction step with the tracking from $\z_t$. Therefore, if we are interested to use another predictive model, the shown KF reformulation can be adopted to incorporate the a priori predictor of $\x_t$ into the measurements $\z_t$. For the GP-VAR, for instance, the $\P_t^-$ can be derived from \eqref{eq.gcp_MSE2}.
%
%In the above tracking analysis, an important role is played by the $K$-rank decomposition of $b_0(\L_\Gr)$, which connects the prediction from the past data with the collected measurements. The later is an intrinsic part of the G-VARMA model which rendered the above tracking analysis more easy to be derived. If one opts for the GP-VAR model \eqref{eq.gcp_varma} or the RGP-VAR model from \cite{mei2017signal} the link of predicted signal with the measurements at time $t$ is not anymore given by $b_0(\L_\Gr)$ (which is the identity matrix), but from their prediction covariance matrices (i.e., $P_t^-$).
\end{remark}

%\begin{remark} In the prediction of $\tilde{\x}_{\Scal_c,t}$ in \eqref{eq.gc_varma_subgr4}, we note that an important role is played by the $K$-rank decomposition of $b_0(\L_\Gr)$. The latter connects the signal to be predicted in $\Scal_c$ with the sampled nodes on $\Scal$ and the past history of the data. Therefore, for the predictors where $b_0(\L_\Gr) = \I_N$ the subgraph prediction becomes a challenging task. This is the case of the CGP-VAR and RCGP-VAR  \cite{mei2017signal} predictors that do not contain the MA part in their model. 
%\end{remark}








